XraySyn: Realistic View Synthesis From a Single Radiograph Through CT Priors

A radiograph visualizes the internal anatomy of a patient through the use of X-ray, which projects 3D information onto a 2D plane. Hence, radiograph analysis naturally requires physicians to relate the prior about 3D human anatomy to 2D radiographs. Synthesizing novel radiographic views in a small range can assist physicians in interpreting anatomy more reliably; however, radiograph view synthesis is heavily ill-posed, lacking in paired data, and lacking in differentiable operations to leverage learning-based approaches. To address these problems, we use Computed Tomography (CT) for radiograph simulation and design a differentiable projection algorithm, which enables us to achieve geometrically consistent transformations between the radiography and CT domains. Our method, XraySyn, can synthesize novel views on real radiographs through a combination of realistic simulation and finetuning on real radiographs. To the best of our knowledge, this is the first work on radiograph view synthesis. We show that by gaining an understanding of radiography in 3D space, our method can be applied to radiograph bone extraction and suppression without groundtruth bone labels.

==> XraySyn New/abstract.tex <==
\begin{abstract}

X-ray view synthesis has seldom been studied compared to its natural image counterpart due to various prohibitive challenges. Firstly, multi-view X-ray images are rare due to the invasive acquisition process, and X-ray simulations are either unrealistic or computationally expensive. Secondly, the material-penetrating nature of X-ray means that synthesizing from different views requires 3D knowledge of both the surface and internal of the subject. Lastly, as materials attenuate differently, dense but small details such as bones have a large impact on synthesized X-ray images but are hard to generate realistically. In this work, we conceive a differentiable projectior algorithm, named CT2Xray, to efficiently generate realistic X-ray simulations from CT volumes, thus resolving the first challenge. We also propose an end-to-end X-ray view synthesis algorithm called $\textit{XraySyn}$, which is able to synthesize X-ray views with high realism. We further show that XraySyn performs robustly on real X-ray images without extra steps for domain adaptation. To the authors' best knowledge, this is the first work on realistic X-ray image view synthesis. Code will be made available on GitHub.



\end{abstract}

==> XraySyn New/abstract_new.tex <==
\begin{abstract}
\footnotetext[1]{Equal contribution. Cheng proposed and implemented the XraySyn framework for view synthesis and bone suppression, labeled data, and performed relevant experiments. Haofu initiated the project, proposed and implemented the differentiable forward/backprojector module, and provided valuable discussions.}
A radiograph visualizes the internal anatomy of a patient through the use of X-ray, which projects 3D information onto a 2D plane. Hence, radiograph analysis naturally requires physicians to relate the prior about 3D human anatomy to 2D radiographs. Synthesizing novel radiographic views in a small range can assist physicians in interpreting anatomy more reliably; however, radiograph view synthesis is heavily ill-posed, lacking in paired data, and lacking in differentiable operations to leverage learning-based approaches. To address these problems, we use Computed Tomography (CT) for radiograph simulation and design a \textbf{differentiable projection} algorithm, which enables us to achieve geometrically consistent transformations between the radiography and CT domains. Our method, XraySyn, can synthesize novel views on \textbf{real radiographs} through a combination of realistic simulation and finetuning on real radiographs. To the best of our knowledge, this is \textbf{the first work} on radiograph view synthesis. We show that by gaining an understanding of radiography in 3D space, our method can be applied to radiograph bone extraction and suppression without groundtruth bone labels.



% A radiograph visualizes the internal of a patient through the use of X-ray, which projects 3D information onto a 2D plane. Hence, radiograph analysis requires physicians to relate the strong prior about human anatomy in 3D to the 2D radiograph plane. However, radiograph analysis algorithms so far have mostly forgone the task of relating radiograph to 3D space, due to its heavily ill-posed nature and a lack of paired data. 
% We tackle this problem in the form of novel view synthesis from a \emph{single} radiograph. To accomplish this, we leverage Computed Tomography (CT) for radiograph simulation to address the estimation of 3D human anatomy. In particular, we conceive a \textbf{differentiable projection} algorithm, which enables us to achieve geometrically consistent transformations between the radiography and CT domain. %, and hence improves performance of such transformations as approximated by CNNs. 
% Furthermore, our method, XraySyn, can synthesize novel views on \textbf{real radiographs} through a combination of realistic radiograph simulation and self-supervised learning. To the best of our knowledge, this is \textbf{the first work} on radiograph view synthesis. By gaining an understanding of radiography in 3D space, our work enables different avenues for designing radiograph analysis algorithms. We show how our method can be applied to bone extraction on radiographs without groundtruth labels.

\end{abstract}

==> XraySyn New/conclusion.tex <==
\section{Conclusion}
We propose a two-stage radiograph view synthesis method, XraySyn. This method estimates a coarse 3D CT from a 2D radiograph, simulates a novel view from the estimated volume, and finally refines the views to be visually consistent with real radiographs. The learning process of XraySyn is enabled by our proposed differentiable forward projector and backprojector. Furthermore, by incorporating the CT bone labels in CT2Xray that is inspired by DeepDRR and implemented with our differentiable forward projector, we not only achieve realistic simulation for training the radiograph-to-CT transformation, but also gain the ability to transfer bone labels from CT to radiograph. We carefully evaluate our method both on simulated and real radiographs, and find that XraySyn generates highly realistic and consistent novel view radiographs. To the best of our knowledge, this is the first work on radiograph view synthesis, which can help give practitioners a more precise understanding of the patient's 3D anatomy. XraySyn also opens up possibilities for many downstream processes on radiograph, such as lesion detection, organ segmentation, and sparse-view CT reconstruction. Currently, XraySyn is limited in resolution due to memory constraint of 3DPN. We plan to address this limitation through a more efficient network design. In addition, we will conduct a study to assess the effect of bone suppression for clinical diagnosis.

%One limitation of XraySyn is that the synthesized novel view can not deviate from the input view by a large margin. Currently we perform our experiment with $\pm18\degree$. In future, we plan to address the above limitation say by introducing more fiducial views. In addition, we will conduct a study to assess the effect of bone suppression for clinical diagnosis.

% In this work, we tackle the X-ray view synthesis problem, which has been relatively unexplored due to the difficulties in establishing correspondence between 2D X-ray images and their 3D counterparts. To solve this issue, we first propose a CT2Xray projection algorithm that can realistically simulate X-ray images from CT volumes. The algorithm is differentiable, which enables end-to-end training between the X-ray and CT modalities. We further propose XraySyn, a novel end-to-end algorithm for X-ray view synthesis, to recover high quality CT volumes from X-ray images. We carefully evaluate our method both on simulated and real X-ray images, and find that XraySyn can generate highly realistic alternative views of imaged object. While the current method is still somewhat constrained by limited dataset and hyperparameters, we believe these problems can be addressed through subsequent research, and that this work shows promising advance towards real applications.



==> XraySyn New/experiment.tex <==
\section{Experiments}

\input{tables/newer_ablation}

\subsubsection{Implementation details}
The two stages of XraySyn are trained separately. To train 3DPN, a CT volume $V_{\textrm{gt}}$ and its bone mask $V^{\textrm{gt}}_{\textrm{mask}}$ is used to simulate the groundtruth radiographs $I^{T}_{\textrm{in}}$ and $I^{T^{'}}_{\textrm{gt}}$. $T$ and $T^{'}$ are sampled randomly from -18$\degree$ to 18$\degree$ in azimuth and elevation angles. During the training of 2DRN, real radiographs are used as $I^{T}_{in}$ in place of simulated radiographs, and the 3DPN's parameters are frozen. Furthermore, the input is first downsampled through average pooling as real radiographs are of higher resolution. As view angles are not available for real radiographs, we sample $T$ and $T^{'}$ randomly in similar fashion as for 3DPN training. For testing on real radiograph, $T$ is assumed to be the canonical frontal view, $T^{'}$ are twenty view angles uniformally spaced from -9$\degree$ to 9$\degree$ in azimuth. Due to the discretization of the voxel-based representation, the ray tracing process used in forward and backprojection needs to approximate points in space when those points are not on the coordinate grid. We use trilinear interpolation for such approximation. The networks are implemented with Pytorch, and trained using four Nvidia P6000 GPUs for five days. The details of network structure are reported in the supplemental material. 

 
% As shown in Figure. 2, at each training iteration, a CT volume $V_{CT}$ is used to simulate the groundtruth X-ray images from view rotations $T, T^{'}$. All simulated X-ray images generated from the CT2Xray operator are normalized to range between 0 and 1. We find thresholding to be the most robust method to separate bone and tissues in any given CT volume, as well as computationally inexpensive. For simulation during training, we randomly select the hyperparameter $\omega_{tissue}$ to be between 0.8 to 1.2 and clip the dynamic range of the generated $I_{Xray}$ from 70 to 100$\%$ to simulate for different real X-ray images. We further select $T$ and $T^{'}$ randomly from -18$\degree$ to 18$\degree$ in azimuth and elevation angles. For simulation during testing, $\omega_{tissue}$ is set to be 0.8, and image dynamic range is clipped at 90$\%$. We set $\lambda_{in} = 1.0$ and $\lambda_{new} = 0.25$ for $\mathcal{L}^{G, F}_{xray}$, and $\lambda_{CT} = \lambda_{xray} = 1.0$. Due to the discretization of a voxel-based representation in digital system, the ray tracing process used in forward and backprojection can only approximates points in space when those points are not on integer coordinates. We use trilinear interpolation for such approximation. For more details about implementation, please refer to the supplemental material.


\subsubsection{Dataset}
Both CT and radiograph datasets are needed for training XraySyn. To train the 3DPN, we use the LIDC-IDRI dataset \cite{armato2011lung}, which contains
1,018 chest CT volumes. We discards all volumes that have a between-slices resolution higher than 2.5mm. This leads to 780 CT volumes, from which we randomly select 700 for training, 10 for evaluation, and 70 for testing. To preprocess the data, we tightly crop the CT volumes to eliminate excess empty space, and reshape the volumes into resolution of $128\times128\times128$. To train 2DRN with real radiographs, we use the TBX11K dataset \cite{DBLP:conf/cvpr/LiuWBWC20}. Specifically, to avoid the excessive interference of foreign objects and abnormal anatomy, we manually select 3000 images under the healthy category within TBX11K and crop those images to have similar field-of-view as the CT simulation. The images are then reshaped to resolution of $256\times256$. We randomly select 2600 for training, 100 for evaluation, and 300 for testing.


% resample the CT volumes to a uniform voxel resolution of $2\times2\times2\textrm{mm}^3$ and crop a central region of $256\times256\times256\textrm{mm}^3$ from each CT scan.


% As there exists no public dataset that contains either aligned, multi-view X-ray data, or geometrically paired X-ray and CT data, we use CT volumes and our proposed CT2Xray operator to simulate these relationships. Specifically, we use the LIDC-IDRI dataset \cite{armato2011lung}, which contains
% 1,018 chest CT volumes, for simulation. To preprocess the LIDC-IDRI data, we resample the CT volumes to a uniform voxel resolution of $2\times2\times2\textrm{mm}^3$ and crop a central region of $256\times256\times256\textrm{mm}^3$ from each CT scan. Furthermore, we discards all volumes that have a between-slices resolution higher than 2.5mm. This leads to 780 CT volumes, where we randomly select 700 for training, 10 for evaluation, and 70 for testing. To show the robustness of our method on real images, we select a number of suitable X-ray images from CheXpert \cite{DBLP:conf/aaai/IrvinRKYCCMHBSS19} for testing.


%  As shown in Figure. 2, such simulation is done at online training, where the only required input

%Proper preprocessing steps, such as rotating and cropping, are taken to ensure the real X-ray images are geometrically similar with simulated X-ray images from the training dataset.

%explain the experiment setup as simulations, i.e. the entire pipeline



\subsubsection{Evaluation metrics}
Evaluation of novel view synthesis on real radiograph can be challenging, as there is no groundtruth. Therefore, we first provide the results of evaluation on simulated radiographs. Peak Signal-to-Noise Ratio (PSNR) and Structured Similarity Index (SSIM) \cite{DBLP:journals/tip/WangBSS04} are used to measure the quality of synthesized novel views and material decomposition. For real radiographs, we use PSNR and SSIM to measure the quality of reconstruction for the input view $T$ and Fréchet Inception Distance (FID) \cite{DBLP:conf/nips/HeuselRUNH17} to measure the realism of the novel view radiograph in comparison to the input view radiograph. Since radiographs are grayscale images, we do the following to adapt to the ImageNet-trained InceptionV3 model: 1) we repeat the grayscale values across the RGB channels, and 2) use the middle layer features from InceptionV3, specifically the 768-channel layer before InceptionV3’s last auxiliary classifier, for better generalizability.


% There are several different factors involved with evaluating the effectiveness of X-ray view synthesis. Firstly, as the input X-ray image is the only reliable data about the subject, one goal is to ensure that such information is preserved during the proposed 2D-to-3D inversion. To this end, we use Peak Signal-to-Noise Ratio (PSNR) and Structured Similarity Index (SSIM) to measure the overall recovery of the input X-ray image. To address the aspect of recovering realistic anatomical details, we measure the PSNR/SSIM value of $t(tissue)$ and $t(bone)$ for the input and output X-ray images of the same view. Lastly, Fréchet Inception Distance (FID) is used as a metric to measure realism of the generated X-ray images. We make two adaptions to FID for X-rays: 1. repeating the grayscale values across the RGB channels as the pre-trained InceptionV3 model works on RGB images; 2. calculating the FID score by using the middle layers of InceptionV3, specifically the 768-channel layer before InceptionV3's last auxiliary classifier, for lower level features. The same evaluation metrics are calculated for synthesized views over a set of 10 angles, which are uniformly selected -18$\%$ to 18$\%$ azimuthally from the input view angle. 


\input{imgs/ablation_sim}
\subsubsection{Ablation study}
We evaluate the effectiveness of XraySyn against alternative 2D or 3D methods. Firstly, comparisons against 3DPN are made under simulated setting for the following setups: 
\begin{itemize}
%\begin{enumerate}[label=\Alph*),itemsep=1 pt]
    \item 2D Refiner: An image-to-image method by synthesizing new views from input $\textrm{FP}(\textrm{BP}(I^{T}_{\textrm{in}}, T),T^{'})$ through a 2D DenseNet structure. The training is constrained by a L1 loss between the generated X-ray and its groundtruth. 
    % \item 2D Encoder: A 2D DenseNet structure that directly projects $I^{T}_{in}$ onto the latent space of the chest CT PGGAN.The training losses are consistent with Eq. \ref{eqn:loss+} with $\lambda_{CT}=1.0$, $\lambda_{Xray}=0.25$, and no $\mathcal{L}_{code}$. 
    \item X2CT: Proposed by Ying et al. \cite{DBLP:conf/cvpr/YingGMWWZ19} to transform DRRs into CT volumes. We made the following adaptations: (i) instead of DRRs, the inputs are X-rays generated by CT2Xray, and (ii) the training losses are consistent with Eq. (\ref{eqn:loss3dpn}).
    \item 3DPN-DRR: An alternative 3DPN that directly uses forward projection to simulate radiographs, i.e. DRRs. Note that no material decomposition is involved in DRR.
%\end{enumerate}
\end{itemize}
Comparisons against the overall XraySyn method are then made for generating real radiographs. These include:
\begin{itemize}%[label=\Alph*),itemsep=1 pt]
    \item 3DPN: A direct use of 3DPN trained on simualted data.
    \item $\textrm{XraySyn}^{\textrm{no}\mathcal{M}}$: An alternative XraySyn where the 2DRN stage does not have $\mathcal{M}$.
\end{itemize}

% 1. directly using 3DPN on real radiographs, 2. using an XraySyn alternative where 2DRN does not have the filter generating $\mathcal{M}$ component.


Table \ref{tab:ablation_table} summarizes the performance of different implementations over various view angles, and visualization of the results are provided in Fig. \ref{tab:ablation_img}. Image-to-image approach like 2D Refiner synthesizes mostly a blurry version of the input view. The lack of an explicit 3D loss forces the network to overly smooth the output for the best PSNR. The implementation of X2CT-CNN copies the 2D features along a third axis to achieve the initial upsampling from 2D to 3D, which is geometrically incorrect for arbitrary view angle. While CNN's strong learning ability still helps X2CT-CNN produce a coarse 3D estimation, it has difficulty in learning the geometric transformation that maps the input image to the correct view. Consequently, the synthesized views are reliant on a poorly estimated 3D structure and lack significant details, specifically over the rib cage area. 
\input{imgs/ablation_real_updated}
By using the geometrically consistent backprojection and forward projection, 3DPN-DRR and 3DPN perform much better at preserving the input radiograph during the 2D-to-3D transformation. The main issue of DRR is its assumption that the rays attenuate over bone and tissue similarly, when in fact bone attenuates X-Rays much better and therefore has better contrast on real radiographs. The results show that when 3DPN-DRR is used on more realistically simulated radiographs, bone appears much softer. While this impacts PSNR significantly, 3DPN-DRR results have much better SSIM scores compared to X2CT and 2D Refiner due to the superior 3D estimation. Finally, 3DPN, which includes all proposed components, performs much better than other methods (6-7dB more than the second best method in terms of PSNR) at capturing the 3D anatomy from a single radiograph. As 2D-to-3D transformation is still ill-posed, the metrics worsen when the novel view is further from the input view. Please see the supplementary material section for more detailed metrics.

Using 3DPN to perform view synthesis on real radiographs involves additional challenges. Specifically, 3DPN is limited in the available resolution and cannot generate sufficient details, e.g. as shown in Fig. \ref{tab:ablation_img_real}, 3DPN-generated bone structure is less visible on the rib cage area, as those bones are small and hard to be accurately estimated in 3D. Furthermore, simulation does not address complex imaging conditions. As a result, views synthesized through 3DPN are blurry and constrained to have a certain image style due to the formulation of CT2Xray. 2DRN is proposed to address these problems by performing refinement on $t^{\textrm{CT}}_{m}(T^{'})$ to preserve the material decomposition information. 

After refining the 3DPN results in $\textrm{XraySyn}^{\textrm{no}\mathcal{M}}$, the novel views are much improved in both low-level details and overall realism, along with the corresponding bone map $t^{\textrm{ref}}_{\textrm{bone}}$. However, some information is inevitably lost during 3DPN. The input in Fig. \ref{tab:ablation_img_real} is grayish in the lung area, as opposed to the typical dark color from simulation. This information is not captured in 3DPN, thus the subsequent refinement network is also limited in its recovery performance. $\mathcal{M}$ is designed to shuffle information directly from the input radiograph. To prevent 2DRN from learning an identity transform of the input radiograph, $\mathcal{M}$ generates convolutional filter parameters to constrict the information flow. The complete XraySyn, which includes $\mathcal{M}$ in 2DRN, improves the overall performance \input{imgs/suppress}by almost 1dB with little additional computational cost. While 2DRN does not explicitly guarantee overall 3D consistency, we observe that the novel views are fairly consistent with each other due to the residual learning on the 3D-consistent 3DPN results. As the refinement on $t^{\textrm{CT}}_{m}$ is not directly supervised, we observe a slight amount of background noise despite training the network with a residual connection. However, this can be addressed through post-processing steps. It is worth noting that due to the lack of alternative-view radiograph dataset, synthesized novel views beyond a limited range from the frontal view may lead to unfaithful results as compared to real circumstances.

% is not advised deviate from the input view by a large margin

% The synthesized novel view cannot deviate from the input view by a large margin due to lack of alternative-view real radiograph data.

% while XraySyn can synthesize to wider range of views, as real radiographs 

\subsubsection{Bone suppression}
A natural application of XraySyn is on radiograph bone suppression, which seeks to reduce bone attenuation and better reveal the underlying tissues. To best preserve the tissue information from input radiograph $I^{T}_{\textrm{in}}$, we find $t^{\textrm{ref}}_{\textrm{bone}}$ and $t^{\textrm{recon}}_{\textrm{tissue}}$ so that they losslessly reconstruct $I^{T}_{\textrm{in}}$, through reversing the CT2Xray operation as shown in Eq. (\ref{eq:ct2xray_eq}). In Fig. \ref{fig:suppress}, we show that our approach suppresses most of the rib cage bones while preserving the tissue content. For a mathematical formulation on reversing CT2Xray, please refer to the supplemental material section. 


% To accomplish bone suppression as a post process, we need to perform an inversion of CT2Xray to reduce bone attenuation and preserve the tissue content based on the original input, as $t^{\textrm{ref}}_{\textrm{tissue}}$ may be prone to error. There are two summation operations in CT2Xray that confound information, as shown in Eq. \ref{eq:ct2xray_eq}. To address this issue, we 1) normalize the range of input radiograph $I^{T}_{\textrm{in}}$, which is stored in an image format, to the range of $I^{T}_{\textrm{atten}}$, as calculated during the reconstruction of $I^{T}_{\textrm{in}}$ in 2DRN, 2) use $t^{\textrm{ref}}_{\textrm{bone}}$ and $t^{\textrm{ref}}_{\textrm{tissue}}$ as references to calculate the proportions of different terms in the summation operations, and 3) use $I^{T}_{\textrm{in}}$ and $t^{\textrm{ref}}_{\textrm{bone}}$ to calculate a $t^{\textrm{recon}}_{\textrm{tissue}}$ such that $t^{\textrm{ref}}_{\textrm{bone}}$ and $t^{\textrm{recon}}_{\textrm{tissue}}$ losslessly reconstructs $I^{T}_{\textrm{in}}$. Finally, we reduce the attenuation of $t^{\textrm{ref}}_{\textrm{bone}}$ in Eq. (\ref{eq:ct2xray_eq}) and produce a bone-suppressed radiograph, as shown in Fig. \ref{fig:intro}. For a more comprehensive mathematical formulation, please refer to the supplemental material.

% 2DRN refines on $t^{CT}_{m}$ instead of on radiographs to preserve the material decomposition information. Similar to novel views, $t^{CT}_{m}$ lacks direct groundtruth to be learned from. 3DPN-generated bone structure, as shown in Fig. \ref{tab:ablation_img_real}, is less accurate on smaller bones such as the rib cage, as those bones are hard to be accurately predicted in 3D. After the refinement through 2DRN, the bone structure is much more complete with respect to the input radiograph. There is a slight amount of background noise in $t^{ref}_{m}$ as compared to $t^{CT}_{m}$, as 

% we can see that XraySyn not only reproduces the detailed anatomy, but also matches the grayish overall style.



% CT2Xray does not account for the complex imaging condition, e.g. depending on the number of photons and their energy state, two radiographs of the same person can have very different contrast. The variation of such 2D imaging condition is hard to be accounted for in a purely 3D representation. As shown in Fig. \ref{tab:ablation_img_real}, views synthesized through 3DPN are both blurry and have a different contrast than the input radiograph. 


% 3DPN also performs sub-optimally on real radiograph in terms of resolution and image quality, as shown in Fig. \ref{tab:ablation_img_real}


% XraySyn and XraySyn+ excel in preserving the input X-ray view in their generated CT volume. Specifically, we examine XraySyn with different loss setups to observe the utility of each loss component. $\textrm{XraySyn}^{v1}$ is trained with only $\mathcal{L}^{G}_{CT}$ to best approximate the original CT volume. Due to the ill-posed nature of 2D-to-3D conversion, however, the generated CT volume can still be very different from the groundtruth, as shown in Fig. \ref{tab:ablation_img}. By adding the $\mathcal{L}^{G}_{xray}$ term in training $\textrm{XraySyn}^{v2}$, we explicitly enforces the preservation of the input X-ray view, which leads to significantly better synthesized images metrically and visually, specifically on the recovery of bone structures. We further observe that both results from $\textrm{XraySyn}^{v1}$ and $\textrm{XraySyn}^{v2}$ are lacking in a realistic bone structure, which is also evident in CT. $\textrm{XraySyn}^{v3}$ adds a LSGAN component to the loss formulation to promote more realistic recovery of bone structures. It can be observed that $\textrm{XraySyn}^{v3}$ produces a better bone-tissue contrast in CT, but is unable to reach satisfactory definition in details. Overall, XraySyn performs well at generating the 3D volume that preserves the original X-ray input in terms of PSNR, with some deficiency in generating bone details.

% 
% XraySyn+ is introduced to address this issue. By leveraging the underlying manifold found through 3D PGGAN, XraySyn+ is able to generate realistic CT volume with a clear bone structure. For comparison, an alternative 2D Encoder is implemented to directly projects the input X-ray image onto the chest CT manifold. We find that the lack of auxiliary constraint like $\mathcal{L}_{code}$, along with the limited input information in 2D, leads 2D Encoder to find sub-optimal solutions. XraySyn+ performs much better than 2D Encoder in terms of PSNR/SSIM, while providing much more realistic X-ray images both visually and according to the FID scores. On the other hand, due to various challenges in GAN inversion and the limited data used to train a PGGAN, XraySyn+ is constrained in its ability to produce images that are as pixel-wise consistent as $\textrm{XraySyn}^{v2}$. However, we find the bone and tissue-wise metrics for XraySyn+ and $\textrm{XraySyn}^{v2}$ are much more similar, suggesting that part of the difference in X-ray PSNR/SSIM metrics is due to the the segmentation component in CT2Xray. In general, we find that the imperfections of segmentation methods lead to favorable X-ray PSNR/SSIM measurements for $\textrm{XraySyn}^{v2}$, as the CT volume produced by $\textrm{XraySyn}^{v2}$ is smoother and less noisy when segmented. In comparison PGGAN produced CT volumes are much more detailed and more difficult to segment properly. 

% Lastly, we note that comparisons for synthesized non-input views are difficult. While measurements with respect to views generated from the groundtruth volume can serve as a guidance, they should be considered with the understanding that no method can recover the exact volume since 2D-to-3D inversion is a one-to-many mapping. This demonstrates the difficulties in X-ray view synthesis. In general, we find that XraySyn produces more voxel-wise accurate CT volume and thus pixel-wise accurate X-ray images; however, as the view angle shifts further away from the input view, more bone structure may be missing. In contrast, XraySyn+ produces less voxel-wise accurate CT volume, but realistic X-ray images regardless of the view angle.

% \subsection{XraySyn+ on Real X-ray Images}
% In this section, we exam XraySyn+'s performance on real X-ray images. There are many hyperparameters related to view synthesis, including the unknown input view angle $T$, the distance between X-ray source to detector, the dynamic range of the X-ray images, etc. To accurately estimate these hyperparameters is out of the scope of this paper. In this paper, we roughly estimate these hyperparameters by 1. cropping and rotating the original X-ray image into regions that are similar to the training dataset, and 2. search through a small interval of view transform $T$ on the output CT to find a $T$ that achieves the highest PSNR value between the generated and observed X-ray image. 

% Fig. \ref{img:real_results} shows the visual results of XraySyn+ on real X-ray images. As we can see, XraySyn+ does a fairly good job at preserving the overall anatomy, indicating that simulated X-ray images generated through CT2Xray are effective at capturing X-ray characteristics. The new views can provide users with knowledge of how organs, e.g. the heart and lung, are shaped in 3D. We observe that there are some discrepancies between real and generated X-ray images, especially at the lower, abdominal section where shadows in the real X-ray images are not represented. This may be due to 1. the abdominal section is not well represented in the limited chest CT dataset, and 2. the material in the abdominal section is not well modelled in CT2Xray. As the training dataset expands to cover more human anatomy and better separation at different materials, we posit that the results will be much improved. 



==> XraySyn New/experiment_backup.tex <==
\section{Experiments}

\input{tables/modified_ablation}
\subsection{Dataset}
As there exists no public dataset that contains either aligned, multi-view X-ray data, or geometrically paired X-ray and CT data, we use CT volumes and our proposed CT2Xray operator to simulate these relationships. Specifically, we use the LIDC-IDRI dataset \cite{armato2011lung}, which contains
1,018 chest CT volumes, for simulation. To preprocess the LIDC-IDRI data, we resample the CT volumes to a uniform voxel resolution of $2\times2\times2\textrm{mm}^3$ and crop a central region of $256\times256\times256\textrm{mm}^3$ from each CT scan. Furthermore, we discards all volumes that have a between-slices resolution higher than 2.5mm. This leads to 780 CT volumes, where we randomly select 700 for training, 10 for evaluation, and 70 for testing. To show the robustness of our method on real images, we select a number of suitable X-ray images from CheXpert \cite{DBLP:conf/aaai/IrvinRKYCCMHBSS19} for testing.


%  As shown in Figure. 2, such simulation is done at online training, where the only required input

%Proper preprocessing steps, such as rotating and cropping, are taken to ensure the real X-ray images are geometrically similar with simulated X-ray images from the training dataset.

%explain the experiment setup as simulations, i.e. the entire pipeline

\subsection{Implementation Details}
As shown in Figure. 2, at each training iteration, a CT volume $V_{CT}$ is used to simulate the groundtruth X-ray images from view rotations $T, T^{'}$. All simulated X-ray images generated from the CT2Xray operator are normalized to range between 0 and 1. We find thresholding to be the most robust method to separate bone and tissues in any given CT volume, as well as computationally inexpensive. For simulation during training, we randomly select the hyperparameter $\omega_{tissue}$ to be between 0.8 to 1.2 and clip the dynamic range of the generated $I_{Xray}$ from 70 to 100$\%$ to simulate for different real X-ray images. We further select $T$ and $T^{'}$ randomly from -18$\degree$ to 18$\degree$ in azimuth and elevation angles. For simulation during testing, $\omega_{tissue}$ is set to be 0.8, and image dynamic range is clipped at 90$\%$. We set $\lambda_{in} = 1.0$ and $\lambda_{new} = 0.25$ for $\mathcal{L}^{G, F}_{xray}$, and $\lambda_{CT} = \lambda_{xray} = 1.0$. Due to the discretization of a voxel-based representation in digital system, the ray tracing process used in forward and backprojection can only approximates points in space when those points are not on integer coordinates. We use trilinear interpolation for such approximation. For more details about implementation, please refer to the supplemental material.


\subsection{Evaluation Metrics}
There are several different factors involved with evaluating the effectiveness of X-ray view synthesis. Firstly, as the input X-ray image is the only reliable data about the subject, one goal is to ensure that such information is preserved during the proposed 2D-to-3D inversion. To this end, we use Peak Signal-to-Noise Ratio (PSNR) and Structured Similarity Index (SSIM) to measure the overall recovery of the input X-ray image. To address the aspect of recovering realistic anatomical details, we measure the PSNR/SSIM value of $t(tissue)$ and $t(bone)$ for the input and output X-ray images of the same view. Lastly, Fréchet Inception Distance (FID) is used as a metric to measure realism of the generated X-ray images. We make two adaptions to FID for X-rays: 1. repeating the grayscale values across the RGB channels as the pre-trained InceptionV3 model works on RGB images; 2. calculating the FID score by using the middle layers of InceptionV3, specifically the 768-channel layer before InceptionV3's last auxiliary classifier, for lower level features. The same evaluation metrics are calculated for synthesized views over a set of 10 angles, which are uniformly selected -18$\%$ to 18$\%$ azimuthally from the input view angle. 


\input{imgs/ablation}
\subsection{Ablation Study}
We evaluate the effectiveness of XraySyn 1. against alternative 2D or 3D implementations, and 2. over different training loss setups. Specifically, comparisons are made between the following setups: 

\begin{enumerate}[label=\Alph*),itemsep=1 pt]
    \item 2D Refiner: A baseline image-to-image method by synthesizing new views from input $FP(BP(I^{T}_{in}, T),T^{'})$ through a 2D DenseNet structure. The training is constrained a L1 loss between the generated X-ray and its groundtruth. 
    \item 2D Encoder: A 2D DenseNet structure that directly projects $I^{T}_{in}$ onto the latent space of the chest CT PGGAN.The training losses are consistent with Eq. \ref{eqn:loss+} with $\lambda_{CT}=1.0$, $\lambda_{Xray}=0.25$, and no $\mathcal{L}_{code}$. 
    \item X2CT-CNN: Proposed by Ying et al. to transform DRRs into CT volumes. We made the following adaptations: 1. instead of DRRs, the inputs are X-rays generated by CT2Xray, and 2. the training losses are consistent with Eq. \ref{eqn:loss}, where $\lambda_{CT}=1.0$, $\lambda_{Xray}=0.25$, $\lambda_{GAN}=0.0$;
    \item $\textrm{XraySyn}^{v1}$: XraySyn with $\lambda_{CT}=1.0$, $\lambda_{Xray}=0.0$, $\lambda_{GAN}=0.0$;
    \item $\textrm{XraySyn}^{v2}$: XraySyn with $\lambda_{CT}=1.0$, $\lambda_{Xray}=0.25$, $\lambda_{GAN}=0.0$;
    \item $\textrm{XraySyn}^{v3}$: XraySyn with $\lambda_{CT}=1.0$, $\lambda_{Xray}=0.25$, $\lambda_{GAN}=0.01$;
    \item XraySyn+: XraySyn+ with $\lambda_{CT}=1.0$, $\lambda_{Xray}=0.25$, $\lambda_{code}=0.1$.
\end{enumerate}


Table \ref{tab:ablation_table} summarizes the performance of different implementations over various view angles, visualization of the results are provided in Fig. \ref{tab:ablation_img}. As shown, image-to-image approach like 2D Refiner generates synthesized view as mostly a blurry version of the input view. The lack of an intermediary 3D structure forces the network to account for the variations by overly smoothing the output to achieve a lowest pixel-wise loss. X2CT-CNN copies the features in 2D along the third axis to achieve the initial upsampling from 2D to 3D, which is geometrically incorrect for arbitrary view angle. While we find that CNN's strong curve-fitting ability still leads X2CT-CNN to produce reasonable 3D estimation, it cannot learn the complex geometric transformation that maps the input image to the correct view; therefore, the synthesized views are entirely reliant on the 3D structure and lack significant details, as shown in Fig. \ref{tab:ablation_img}. 

We show that by using the geometrically consistent backprojection and CT2Xray operators, XraySyn and XraySyn+ excel in preserving the input X-ray view in their generated CT volume. Specifically, we examine XraySyn with different loss setups to observe the utility of each loss component. $\textrm{XraySyn}^{v1}$ is trained with only $\mathcal{L}^{G}_{CT}$ to best approximate the original CT volume. Due to the ill-posed nature of 2D-to-3D conversion, however, the generated CT volume can still be very different from the groundtruth, as shown in Fig. \ref{tab:ablation_img}. By adding the $\mathcal{L}^{G}_{xray}$ term in training $\textrm{XraySyn}^{v2}$, we explicitly enforces the preservation of the input X-ray view, which leads to significantly better synthesized images metrically and visually, specifically on the recovery of bone structures. We further observe that both results from $\textrm{XraySyn}^{v1}$ and $\textrm{XraySyn}^{v2}$ are lacking in a realistic bone structure, which is also evident in CT. $\textrm{XraySyn}^{v3}$ adds a LSGAN component to the loss formulation to promote more realistic recovery of bone structures. It can be observed that $\textrm{XraySyn}^{v3}$ produces a better bone-tissue contrast in CT, but is unable to reach satisfactory definition in details. Overall, XraySyn performs well at generating the 3D volume that preserves the original X-ray input in terms of PSNR, with some deficiency in generating bone details.

\input{imgs/real_results}
XraySyn+ is introduced to address this issue. By leveraging the underlying manifold found through 3D PGGAN, XraySyn+ is able to generate realistic CT volume with a clear bone structure. For comparison, an alternative 2D Encoder is implemented to directly projects the input X-ray image onto the chest CT manifold. We find that the lack of auxiliary constraint like $\mathcal{L}_{code}$, along with the limited input information in 2D, leads 2D Encoder to find sub-optimal solutions. XraySyn+ performs much better than 2D Encoder in terms of PSNR/SSIM, while providing much more realistic X-ray images both visually and according to the FID scores. On the other hand, due to various challenges in GAN inversion and the limited data used to train a PGGAN, XraySyn+ is constrained in its ability to produce images that are as pixel-wise consistent as $\textrm{XraySyn}^{v2}$. However, we find the bone and tissue-wise metrics for XraySyn+ and $\textrm{XraySyn}^{v2}$ are much more similar, suggesting that part of the difference in X-ray PSNR/SSIM metrics is due to the the segmentation component in CT2Xray. In general, we find that the imperfections of segmentation methods lead to favorable X-ray PSNR/SSIM measurements for $\textrm{XraySyn}^{v2}$, as the CT volume produced by $\textrm{XraySyn}^{v2}$ is smoother and less noisy when segmented. In comparison PGGAN produced CT volumes are much more detailed and more difficult to segment properly. 

Lastly, we note that comparisons for synthesized non-input views are difficult. While measurements with respect to views generated from the groundtruth volume can serve as a guidance, they should be considered with the understanding that no method can recover the exact volume since 2D-to-3D inversion is a one-to-many mapping. This demonstrates the difficulties in X-ray view synthesis. In general, we find that XraySyn produces more voxel-wise accurate CT volume and thus pixel-wise accurate X-ray images; however, as the view angle shifts further away from the input view, more bone structure may be missing. In contrast, XraySyn+ produces less voxel-wise accurate CT volume, but realistic X-ray images regardless of the view angle.

% While it is expected that metrics like PSNR/SSIM for XraySyn+'s synthesized views are worse compared to $\textrm{XraySyn}^{v2}$, as is often observed in GAN-based super-resolution literature, we find that the bone and tissue-wise metrics for XraySyn+ and $\textrm{XraySyn}^{v2}$ are much more similar. As the generation of X-ray images is based on segmentation of bone and tissues, the pixel-wise consistency between X-ray images is heavily influenced by whether the segmentation outcomes are consistent or not. In general, we find that the imperfections of segmentation methods lead to favorably X-ray PSNR/SSIM measurements for $\textrm{XraySyn}^{v2}$ compared to XraySyn+, as the CT volume produced by $\textrm{XraySyn}^{v2}$ is smoother and less noisy when segmented. Lastly, FID is significantly better for X-ray images generated by XraySyn+ and 2D Encoder, showing that these images are highly realistic. 




% Since X2CT-CNN upsamples 2D image to 3D by repeating the pixel values over the third dimension, the generated volume cannot preserve the original X-ray image and are fully relied on the generated volume. $\textrm{XraySyn}^{Ref}$ generates CT volumes based on $V_{BP}$, which places the X-ray image in 3D according to cone-beam geometry, and has significantly improved performance generating X-ray images over the same view. Despite such a advantage, both methods are unable to generate global details like the bone structure, as is evident in the lateral view. $\textrm{XraySyn}^{Ref}_{GAN}$ adds a GAN Loss to introduce more details in the generated volume; as we can see in Fig. \ref{tab:ablation_img}, constrained by $\mathcal{L}_{CT}$, $\mathcal{L}_{xray}$, and $\mathcal{L}_{GAN}$, $\textrm{XraySyn}^{Ref}_{GAN}$ generates volumes that has mediocre performance in preserving the original X-ray image and generating 3D details. 2D Encoder uses a trained PGGAN to generate 3D Volume, therefore the resulting volume is much more realistic; however, due to the lack of constraint over the latent code and the under-constrained 2D-to-3D condition, 2D Encoder predicts latent codes that are very far away from the normal distribution used to train PGGAN, i.e. gets easily trapped in local minimums. As a result, not only does it underperform during training, 2D Encoder benefits very little from individual fine-tuning. In comparison, XraySyn incorporates the benefits of both $\textrm{XraySyn}^{Ref}$ and 2D Encoder, where it can generate reliable same-view X-ray image, and a highly detailed CT volume.

\subsection{XraySyn+ on Real X-ray Images}
In this section, we exam XraySyn+'s performance on real X-ray images. There are many hyperparameters related to view synthesis, including the unknown input view angle $T$, the distance between X-ray source to detector, the dynamic range of the X-ray images, etc. To accurately estimate these hyperparameters is out of the scope of this paper. In this paper, we roughly estimate these hyperparameters by 1. cropping and rotating the original X-ray image into regions that are similar to the training dataset, and 2. search through a small interval of view transform $T$ on the output CT to find a $T$ that achieves the highest PSNR value between the generated and observed X-ray image. 

Fig. \ref{img:real_results} shows the visual results of XraySyn+ on real X-ray images. As we can see, XraySyn+ does a fairly good job at preserving the overall anatomy, indicating that simulated X-ray images generated through CT2Xray are effective at capturing X-ray characteristics. The new views can provide users with knowledge of how organs, e.g. the heart and lung, are shaped in 3D. We observe that there are some discrepancies between real and generated X-ray images, especially at the lower, abdominal section where shadows in the real X-ray images are not represented. This may be due to 1. the abdominal section is not well represented in the limited chest CT dataset, and 2. the material in the abdominal section is not well modelled in CT2Xray. As the training dataset expands to cover more human anatomy and better separation at different materials, we posit that the results will be much improved. 



==> XraySyn New/imgs/ablation.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}[b]{|ccccccccc|}
        \hline
        View & 2D Refiner & 2D Encoder & X2CT-CNN &  $\textrm{XraySyn}^{v1}$ &$\textrm{XraySyn}^{v2}$ & $\textrm{XraySyn}^{v3}$ &  XraySyn+ & G.T. \\
        Input View & 
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/2d_refiner/2_5_pred.png}
            \caption{22.6/\textbf{0.93}/0.79}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/2d_encoder/2_pred_in.png}
            \caption{18.2/0.61/\textbf{0.48}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/x2ct-cnn/2_pred_in.png}
            \caption{21.9/0.74/2.46}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/3d_only/2_pred_in.png}
            \caption{\underline{24.9}/0.85/1.25}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/unet-l1/2_pred_in.png}
            \caption{\textbf{27.1}/\underline{0.91}/0.92}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/unet-gan/2_pred_in.png}
            \caption{23.9/0.80/1.26}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/xraysyn-refine/2_pred_in.png}
            \caption{24.0/0.78/\underline{0.55}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/2_orig_in.png}
            \caption{\phantom{}}
        \end{subfigure} \\  
        9$\degree$ View & 
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/2d_refiner/2_8_pred.png}
            \caption{22.9/\underline{0.82}/1.87}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/2d_encoder/2_8_pred.png}
            \caption{17.7/0.58/\underline{0.56}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/x2ct/2_8_pred.png}
            \caption{20.7/0.71/2.42}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/xraysyn_v1/2_2_pred.png}
            \caption{\underline{23.2}/0.81/1.11}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/xraysyn_v2/2_8_pred.png}
            \caption{\textbf{24.8/0.85}/1.03}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/xraysyn_v3/2_2_pred.png}
            \caption{22.9/0.78/1.29}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/xraysyn+/2_8_pred.png}
            \caption{22.5/0.76/\textbf{0.43}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/orig/2_8_orig.png}
            \caption{\phantom{}}
        \end{subfigure} \\   
        18$\degree$ View & 
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/2d_refiner/2_10_pred.png}
            \caption{21.2/0.75/2.12}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/2d_encoder/2_pred_gt1.png}
            \caption{16.3/0.56/\underline{0.41}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/x2ct-cnn/2_pred_gt1.png}
            \caption{19.5/0.69/2.51}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/3d_only/2_pred_gt1.png}
            \caption{\underline{22.5}/0.79/0.96}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/unet-l1/2_pred_gt1.png}
            \caption{\textbf{22.8/0.81}/0.88}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/unet-gan/2_pred_gt1.png}
            \caption{20.8/\underline{0.81}/0.88}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/xraysyn-refine/2_pred_gt1.png}
            \caption{20.0/0.73/\textbf{0.33}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/2_orig_gt1.png}
            \caption{\phantom{}}
        \end{subfigure} \\           
        Lateral CT & 
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/blank.png}
            % \caption{14.02/0.3496}
        \end{subfigure} &
        % \diagbox[innerwidth=5em, height=5em]{}{} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/2d_encoder/2_pred_vol.png}
            % \caption{14.02/0.3496}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/x2ct-cnn/2_pred_vol.png}
            % \caption{14.25/0.4601}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/3d_only/2_pred_vol.png}
            % \caption{14.02/0.3496}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/unet-l1/2_pred_vol.png}
            % \caption{15.22/0.4859}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/unet-gan/2_pred_vol.png}
            % \caption{14.19/0.3392}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/xraysyn-refine/2_pred_vol.png}
            % \caption{14.50/0.3902}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/2_orig_vol.png}
            % \caption{PSNR/SSIM}
        \end{subfigure} \\     
        \hline
    \end{tabular}
    \caption{Visual comparisons of X-ray images generated by different methods from different views. View angle change is measured azimuthally. For each non-groundtruth image, PSNR (higher is better), SSIM (higher is better), and FID (lower is better) are provided as metrics. We also provide a lateral image of the generated CT volume for visualization. The best performer is \textbf{bold}, the second best is \underline{underlined}.}
    \label{tab:ablation_img}
\end{figure*}

==> XraySyn New/imgs/ablation_real.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}[b]{|cccccccc|}
        \hline
        View & -9$\degree$ & -6$\degree$ & -3$\degree$ & 0$\degree$ (Input) & 3$\degree$ & 6$\degree$ & 9$\degree$  \\
        3DPN & 
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/xray_pred_0.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/xray_pred_3.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/xray_pred_6.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/xray_pred_10.png}
            \caption{20.80}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/xray_pred_14.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/xray_pred_17.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/xray_pred_20.png}
            \caption{}
        \end{subfigure} \\   
        XraySyn w/o $\mathcal{M}$ & 
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/xray_orig_0.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/xray_orig_3.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/xray_orig_6.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/xray_orig_10.png}
            \caption{22.06}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/xray_orig_0.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/xray_orig_0.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/xray_orig_20.png}
            \caption{}
        \end{subfigure} \\   
        XraySyn & 
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/xray_meta_0.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/xray_meta_0.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/xray_meta_0.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/xray_meta_10.png}
            \caption{29.92}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/xray_meta_14.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/xray_meta_17.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/xray_meta_20.png}
            \caption{}
        \end{subfigure} \\ 
        Groundtruth & 
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/blank.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/blank.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/blank.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xray_orig.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/blank.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/blank.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/blank.png}
        \end{subfigure} \\
        \hline
    \end{tabular}
    \caption{Visual comparisons of X-ray images generated by different methods from different views. View angle change is measured azimuthally. For each non-groundtruth image, PSNR (higher is better), SSIM (higher is better), and FID (lower is better) are provided as metrics. We also provide a lateral image of the generated CT volume for visualization. The best performer is \textbf{bold}, the second best is \underline{underlined}.}
    \label{tab:ablation_img_real}
\end{figure*}

==> XraySyn New/imgs/ablation_real_updated.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}[b]{|cccccccc|}
        \hline
        View & $\textrm{3DPN}_{\textrm{radio}}$ & $\textrm{3DPN}_{\textrm{bone}}$ & $\textrm{XraySyn}^{\textrm{no}\mathcal{M}}_{\textrm{radio}}$ & $\textrm{XraySyn}^{\textrm{no}\mathcal{M}}_{\textrm{bone}}$ & $\textrm{XraySyn}_{\textrm{radio}}$ & $\textrm{XraySyn}_{\textrm{bone}}$ & GT/Input\\
        
        -9$\degree$ & 
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/xray_pred_0.png}
            \caption{0.903}
        \end{subfigure} &
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/bone_pred_0.png}
            \caption{-/-}
        \end{subfigure} &
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/xray_orig_0.png}
            \caption{0.414}
        \end{subfigure} &
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/bone_nocycle_0.png}
            \caption{-/-}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/xray_meta_0.png}
            \caption{\textbf{0.368}}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/bone_refine_0.png}
            \caption{-/-}
        \end{subfigure} &
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/blank.png}
            \caption{FID}
        \end{subfigure} \\
        0$\degree$ & 
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/xray_pred_10.png}
            \caption{23.18/0.832}
        \end{subfigure} &
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/bone_pred_10.png}
            \caption{N/A}
        \end{subfigure} &
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/xray_orig_10.png}
            \caption{24.22/0.845}
        \end{subfigure} &
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/bone_nocycle_10.png}
            \caption{N/A}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/xray_meta_10.png}
            \caption{\textbf{30.60/0.861}}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/bone_refine_10.png}
            \caption{N/A}
        \end{subfigure} &
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xray_orig.png}
            \caption{PSNR/SSIM}
        \end{subfigure} \\        
        9$\degree$ & 
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/xray_pred_20.png}
            \caption{0.929}
        \end{subfigure} &
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/bone_pred_20.png}
            \caption{-/-}
        \end{subfigure} &
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/xray_orig_20.png}
            \caption{0.432}
        \end{subfigure} &
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/bone_nocycle_20.png}
            \caption{-/-}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/xray_meta_20.png}
            \caption{\textbf{0.414}}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/bone_refine_20.png}
            \caption{-/-}
        \end{subfigure} &
        \begin{subfigure}[b]{0.125\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/blank.png}
            \caption{FID}
        \end{subfigure}\\                
        \hline
    \end{tabular}
    \caption{Visual comparisons of novel view radiographs generated by different methods based on real radiographs as inputs. View angle change is measured azimuthally. PSNR/SSIM metrics are provided for input radiograph reconstruction, FID is provided for novel view synthesis with respect to input radiographs. The best metrics are \textbf{bold}. For more results with animation, please refer to the supplemental material.}
    \label{tab:ablation_img_real}
    \vspace{-1.5em}
\end{figure*}

==> XraySyn New/imgs/ablation_sim.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}[b]{|ccccccccc|}
        \hline
        View & 2D Refiner & $\textrm{X2CT}_{\textrm{radio}}$ & $\textrm{X2CT}_{\textrm{bone}}$ & 3DPN-DRR & $\textrm{3DPN}_{\textrm{radio}}$ & $\textrm{3DPN}_{\textrm{bone}}$ & $\textrm{GT}_{\textrm{radio}}$ & $\textrm{GT}_{\textrm{bone}}$\\
        
        % -6$\degree$ & -3$\degree$ & 0$\degree$ (Input View) & 3$\degree$ & 6$\degree$ & 9$\degree$  \\
        -9$\degree$ & 
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/2D/2d_pred_0.png}
            \caption{18.85/0.725}
        \end{subfigure} &
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/X2CT/xray_pred_0.png}
            \caption{\underline{20.70}/0.745}
        \end{subfigure} &
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/X2CT/bone_pred_0.png}
            \caption{17.07/0.470}
        \end{subfigure} &
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/DRR/drr_pred_0.png}
            \caption{19.28/\underline{0.835}}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/3DPN/xray_pred_0.png}
            \caption{\textbf{26.36/0.918}}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/3DPN/bone_pred_0.png}
            \caption{21.47/0.826}
        \end{subfigure} &
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/GT/xray_gt_0.png}
            \caption{PSNR/SSIM}
        \end{subfigure} &
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/GT/bone_pred_0.png}
            \caption{PSNR/SSIM}
        \end{subfigure}\\
        0$\degree$ & 
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/2D/2d_pred_10.png}
            \caption{N/A}
        \end{subfigure} &
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/X2CT/xray_pred_10.png}
            \caption{21.52/0.741}
        \end{subfigure} &
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/X2CT/bone_pred_10.png}
            \caption{16.83/0.470}
        \end{subfigure} &
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/DRR/drr_pred_10.png}
            \caption{\underline{23.26/0.937}}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/3DPN/xray_pred_10.png}
            \caption{\textbf{31.60/0.971}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/3DPN/bone_pred_10.png}
            \caption{23.67/0.872}
        \end{subfigure} &
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/GT/xray_gt_10.png}
            \caption{PSNR/SSIM}
        \end{subfigure}&
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/GT/bone_pred_10.png}
            \caption{PSNR/SSIM}
        \end{subfigure} \\        
        9$\degree$ & 
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/2D/2d_pred_20.png}
            \caption{20.11/0.766}
        \end{subfigure} &
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/X2CT/xray_pred_20.png}
            \caption{\underline{20.54}/0.724}
        \end{subfigure} &
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/X2CT/bone_pred_20.png}
            \caption{15.72/0.397}
        \end{subfigure} &
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/DRR/drr_pred_20.png}
            \caption{20.07/\underline{0.850}}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/3DPN/xray_pred_20.png}
            \caption{\textbf{27.52/0.927}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/3DPN/bone_pred_20.png}
            \caption{22.44/0.817}
        \end{subfigure} &
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/GT/xray_gt_20.png}
            \caption{PSNR/SSIM}
        \end{subfigure} &
        \begin{subfigure}[b]{0.115\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_new_case57/GT/bone_pred_20.png}
            \caption{PSNR/SSIM}
        \end{subfigure}\\                
        \hline
    \end{tabular}
    \caption{Visual comparisons of novel view radiographs generated by different methods based on simulated radiographs as inputs. View angle change is measured azimuthally. For each non-groundtruth image, PSNR/SSIM are provided as metrics. Note that the input view for 2D Refiner is trivially generated as $I^{T}_{in}$. Methods that involve the use of CT2Xray are displayed with both the bone $t^{\textrm{CT}}_{\textrm{bone}}$ and radiograph outputs. The best radiograph generation metrics are \textbf{bold}, the second best is \underline{underlined}.}
    \label{tab:ablation_img}
    \vspace{-1.5em}
\end{figure*}

==> XraySyn New/imgs/intro_img.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\vspace{-5em}
\begin{center}
    \centering
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/xray_meta_0.png}
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/xray_meta_5.png}
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/xray_orig.png}
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/xray_meta_15.png}
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/xray_meta_20.png}\\
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/bone_refine_0.png}
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/bone_refine_5.png}
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/bone_refine_10.png}
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/bone_refine_15.png}
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/bone_refine_20.png}
    % \includegraphics[width=.15\textwidth,height=.15\textwidth]{imgs/intro_img/xray_meta_195.png}
    \captionof{figure}{XraySyn can synthesize novel view radiographs from \emph{real} radiograph inputs, as shown in the first row, where the middle radiograph is the input. In addition, XraySyn also obtains the bone structure within the synthesized views, as shown in the second row. Both synthesized views and their bone structure are generated without direct supervision. For animated results, please refer to the supplemental material.}
\end{center}%
}]

==> XraySyn New/imgs/intro_img_new.tex <==
\begin{figure}[!htb]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}[b]{cc}
        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/intro_img_new_case4/view_orig.png}
            \caption{Input Radiograph}
            \label{input}
        \end{subfigure} &
        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth,height=1\textwidth]{imgs/intro_img_new_case4/view2.png}
            \caption{Synthesized Novel View}
            \label{novel_view}
        \end{subfigure} \\
        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth,height=1\textwidth]{imgs/intro_img_new_case4/bone_proj.png}
            \caption{Bone Estimation on Input}
            \label{bone_est}
        \end{subfigure} &
        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth,height=1\textwidth]{imgs/intro_img_new_case4/xray_suppress.png}
            \caption{Bone Suppression on Input}
            \label{bone_suppress}
        \end{subfigure} \\
    \end{tabular}
    \caption{From (a) a \emph{real} radiograph, XraySyn synthesizes (b) a radiograph of novel view. As the view point rotate clockwise in azimuth angle, observe that the heart and the rib bones, as the blue arrows indicate, change accordingly.
Additionally, XraySyn obtains (c) the bone structure across all views and can be used to perform (d) bone suppression. Both synthesized views and bone estimation are generated without direct supervision. }
    \label{fig:intro}
    \vspace{-1.5em}
\end{figure}

==> XraySyn New/imgs/real_results.tex <==
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}[b]{|cccc|cccc|}
        \hline
        Orig Image & Input View & 18$\degree$ View & 36$\degree$ View & Orig Image & Input View & 18$\degree$ View & 36$\degree$ View\\
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/10_orig.png}
            \caption{Case 1}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/10_input.png}
            \caption{22.08/0.7326}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/10_view1.png}
            \caption{--/--}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/10_view2.png}
            \caption{--/--}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/5_orig.png}
            \caption{Case 2}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/5_input.png}
            \caption{22.31/0.6975}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/5_view1.png}
            \caption{--/--}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/5_view2.png}
            \caption{--/--}
        \end{subfigure} \\
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/7_orig.png}
            \caption{Case 3}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/7_input.png}
            \caption{21.55/0.6943}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/7_view1.png}
            \caption{--/--}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/7_view2.png}
            \caption{--/--}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/23_orig.png}
            \caption{Case 4}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/23_input.png}
            \caption{21.07/0.7099}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/23_view1.png}
            \caption{--/--}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/23_view2.png}
            \caption{--/--}
        \end{subfigure}   \\
        
        \hline
    \end{tabular}
    \caption{View synthesis on real X-ray images. Three views, including the estimated input view and two new views 18$\degree$ and 36$\degree$ azimuthally from the input views are also shown. Some uneven intensity is introduced in alternative views due to the ellipsoid shape of human anatomy. PSNR/SSIM values are provided over the input view.}
    \label{img:real_results}
    \vspace{-1em}
\end{figure*}

==> XraySyn New/imgs/suppress.tex <==
\begin{figure}[!htb]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}[b]{cccc}
        \begin{subfigure}[b]{.24\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/bone_suppression/10/xray_inp.png}
        \end{subfigure} &
        \begin{subfigure}[b]{.24\linewidth}
            \includegraphics[width=\textwidth,height=1\textwidth]{imgs/bone_suppression/7/xray_inp.png}
        \end{subfigure} 
        \begin{subfigure}[b]{.24\linewidth}
            \includegraphics[width=\textwidth,height=1\textwidth]{imgs/bone_suppression/13/xray_inp.png}
        \end{subfigure} &
        \begin{subfigure}[b]{.24\linewidth}
            \includegraphics[width=\textwidth,height=1\textwidth]{imgs/bone_suppression/18/xray_inp.png}
        \end{subfigure} \\
        \begin{subfigure}[b]{.24\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/bone_suppression/10/10.png}
        \end{subfigure} &
        \begin{subfigure}[b]{.24\linewidth}
            \includegraphics[width=\textwidth,height=1\textwidth]{imgs/bone_suppression/7/7.png}
        \end{subfigure} 
        \begin{subfigure}[b]{.24\linewidth}
            \includegraphics[width=\textwidth,height=1\textwidth]{imgs/bone_suppression/13/13.png}
        \end{subfigure} &
        \begin{subfigure}[b]{.24\linewidth}
            \includegraphics[width=\textwidth,height=1\textwidth]{imgs/bone_suppression/18/18.png}
        \end{subfigure} \\    
    \end{tabular}
    \caption{Bone-suppressed radiographs obtained by post-processing the results from XraySyn. (top) Input radiographs from TBX11K \cite{DBLP:conf/cvpr/LiuWBWC20} and (bottom) the bone-suppressed results. Note that the arteries, as indicated with blue arrows, are more visible after bone suppression.}
    \label{fig:suppress}
    \vspace{-2em}
\end{figure}

==> XraySyn New/introduction.tex <==
\section{Introduction}
In the natural image domain, single image view synthesis aims to generate an image of a scene from different viewpoints based on what is observed. Such a task can be formulated as an ill-posed, 2D-to-3D-to-2D problem, and is widely studied in the computer vision and graphics community with the recent advances in Convolutional Neural Networks (CNNs). In general, current single image view synthesis methods can be categorized into two classes, the image-to-image approach and the 3D shape generation approach. Image-to-image methods transform the observed image into an image from a desired view point, either directly or through geometric manipulations. 3D shape generation methods aim to generate a 3D model of the observed object, which can then be rendered from any other viewpoint. Due to the challenging and under-constrained nature of the problem setting, current methods are limited in either the small variability in viewing angle, the detail level of the 3D object, or both.  
%View synthesis has use cases in scene understanding, image editing, and virtual reality. 

Clinical radiographs or X-ray images are formed by applying high energy radiation through the human body, and measuring the attenuated radiation on the other side. The rate of attenuation for every ray yields a pixel value, and in aggregate forms an image that reveals subject's internal anatomy. While X-ray imaging is quick and economic, high energy radiation can cause adverse health effects. As a result, typically only a single X-ray image is taken per session regardless the fact that some radiology readings/analysis may only possible under different views. Therefore, it leads to the need for X-ray view synthesis from a single image, both for clinical use cases and for data-hungry, automated tasks such as X-ray landmark detection, registration, disease identification, etc.


% while 2D-to-3D approaches  
% 3D understanding by generating the desired 3D representation, i.e. 3D shape generation/completion, 2D-3D inversion. Typically, this type of method can only generate surface shape of simple 3D objects.
% and 2. geometrically rotate 2D image based on view angle difference, and compensate the missing information through 2D inpainting [https://arxiv.org/pdf/2004.04727v2.pdf].

Unfortunately, the differences between the imaging physics of X-ray images and natural images make the view synthesis of X-ray images even more challenging than its natural image counterpart. As X-ray can penetrate materials well, the 2D-to-3D inversion step requires the generation of the subject's surface and internal information, which increases the difficulty of the task and renders efficient 3D surface representations such as mesh, point cloud, signed distance function (SDF), etc. inapplicable. Furthermore, due to material-dependent attenuation, small but dense structures like bones are disproportionally represented in X-ray images, which necessitate the inferred 3D information to express fine details. Lastly, as the 2D images are related to a much larger 3D space, small view angle changes lead to significant variation in pixel values, which limits the effectiveness of Image-to-Image methods. These challenges, along with limited data of different views, lead to few works into X-ray view synthesis despite its apparent value. 

Fortunately, there exists a suitable, voxel-based 3D representation that has intrinsic connections to X-ray images. Computational Tomograph (CT), more specifically Cone Beam CT (CBCT), is acquired by measuring 2D X-ray attenuation over many angles and performing 3D reconstruction \cite{Feldkamp:84} to generate a volumetric image. While the 3D reconstruction step is a lossy process, therefore making the relationship between CBCT and X-ray image imprecise, if proper geometric correspondence can be established, the transformation between two domains can be approximated in a data-driven way. We show that our X-ray-to-CT-to-X-ray approach with supervised knowledge in both domains, called XraySyn, can lead to realistic results. To enable application on real data, we take special care to ensure the X-ray simulation is realistic and the resulting models are applicable to real data. In summary, our contribution can be described in four parts:

\begin{enumerate}
    \item We propose a differentiable forward projector called CT2Xray, an operator capable of converting 3D CT to realistically simulated 2D X-rays in real time, therefore providing an efficient solution to establish geometric correspondence between the CT and X-ray domains.
    \item We propose a Unet-based method called XraySyn, which is capable of generating a CT volume based on a single X-ray image. The generated CT is constrained to express the input X-ray image, and can be used to synthesize alternative views.
    \item We propose XraySyn+, which leverages PGGAN to enable realistic generation of detailed anatomical features like the bone structure;
    \item We test our approach on both simulated X-ray images from LIDC \cite{armato2011lung} and real X-ray images from CheXpert \cite{DBLP:conf/aaai/IrvinRKYCCMHBSS19}, and show that it performs robustly on both datasets.
\end{enumerate}









% While the 3D reconstruction step is a lossy process, thereby making the connection between CBCT and X-ray image imprecise, many works have relied on CBCT-generated X-ray simulations, called Digitally Reconstructed Radiographs (DRRs). 




%DRRs are generated by ray tracing through the CBCT volume and summing over the voxel values along the ray, where the voxel values are used as proxies to real attenuation values. 



%While DRRs are computationally inexpensive to generate, they are poor simulations of actual 


% Alternatively, a popular method to simulate X-ray images in silico is based on Computational Tomography, or CT. CT, particularly with cone-beam geometry(CBCT), measures 2D X-ray attenuation of the human body over many angles, and subsequently performs 3D reconstruction\cite{Feldkamp:84} to generate an image of the subject in 3D. As the 3D reconstruction is a lossy process, the connection between CT and X-ray image is imprecise. Regardless, Digitally Reconstructed Radiographs (DRRs) can be generated from CT by projecting the CT voxel values onto a 2D plane in a given direction, and are used as inaccurate but computationally inexpensive X-ray simulations. 





==> XraySyn New/introduction_new.tex <==
\section{Introduction}

Radiography, widely used for visualizing the internal human anatomy, applies high-energy radiation, or X-ray, to pass through the body, and measures the remaining radiation energy on a planar detector. Since different organs attenuate X-ray to various degrees, the detected energy is visualized as a 2D image or a radiograph, that reveals the internal structure of the body and provides valuable diagnostic information. 





% Physicians, who have vast knowledge of the human anatomy, 

% While the overlapping in anatomical features can be somewhat compensated by physicians who have vast knowledge of the human anatomy and can distinguish the different organs on a 2D radiograph in 3D space



\input{imgs/intro_img_new}
Radiography is fast and economical; however, high energy radiation can cause adverse health effects. Conventionally only a single, frontal view radiograph is acquired per session, e.g. for chest radiography. While physicians can intuitively relate the different organs on a 2D radiograph in 3D space, such intuition is implicit and varies in accuracy.  As such, a radiograph view synthesis algorithm can help provide additional information to assist in understanding a patient's internal structure. 
% Such a limitation can be compensated by physicians who have vast knowledge of the human anatomy and intuitively distinguish the different organs on a 2D radiograph in 3D space - although additional views help provide more precise anatomical information. Similar feat is much harder to be accomplished through computerized processes. 
The ability to understand radiographs in a 3D context is also essential beyond providing more visual information. For example, since every pixel on a radiograph represents an X-ray traversing in 3D, it is principally ambiguous to label a pixel as a specific anatomical structure, as X-rays inevitably pass through multiple structures. By exploring 3D context, we can disentangle a pixel into values that represent different structures, and lead to improved analysis algorithms. Particularly, bone extraction on \emph{real} radiographs is difficult, but has been used in fracture analysis \cite{DBLP:journals/corr/abs-2007-01464}, lesion detection \cite{li2020high}, etc. In this work, we tackle radiograph understanding in 3D, specifically through the tasks of novel view synthesis and bone extraction. 

Transforming 2D images to 3D objects is by nature ill-posed. In the natural image domain, deep learning-based methods have shown impressive results in addressing such a problem in a data-driven way. Radiograph view synthesis, however, poses several unique challenges. Firstly, there is no multi-view dataset for radiographs due to privacy and radiation concerns, which prohibits the use of supervised learning. Secondly, there lacks a \emph{differentiable} algorithm that ensures geometrically consistent transformations between radiographs and the 3D space. Lastly, unlike visible light, X-rays can penetrate objects, therefore to inverse the X-ray projection one should take into account both the surface and the internal information in 3D, making the problem even more ill-posed than for natural images and thus poses challenges to unsupervised methods. %In particular, this renders 2D-to-2D view synthesis methods ineffective, as small perturbations in view angle can lead to significant variation in 2D. 

While inverse graphics is a daunting task to be solved directly on real radiographs, some attempts have been made to address it through Digitally Reconstructed Radiographs (DRRs) \cite{DBLP:conf/cvpr/YingGMWWZ19,DBLP:journals/cgf/HenzlerRRR18}. DRRs  \cite{doi:10.1259/bjr/30125639} are simulated radiographs from Computed Tomography (CT) volumes, which are abundantly available. This approach addresses the data scarcity for learning a 2D-3D transformation; however, there remains significant differences between real radiographs and DRRs. The generation of DRRs also cannot be incorporated into a learning-based algorithm, and either is done off-line \cite{DBLP:journals/cgf/HenzlerRRR18} or has severe limitations in available view angles \cite{DBLP:conf/cvpr/YingGMWWZ19}.

%things that didn't get mentioned - leverage CT labels naturally into DeepDRR

In this work, we introduce a novel, two-stage algorithm called \emph{XraySyn} to estimate the 3D context from a radiograph and uses it for novel view synthesis and bone extraction. The first stage of XraySyn, called 3D PriorNet (3DPN), incorporates a pair of differentiable backprojection and forward projection operators to learn the radiograph-to-CT transformation under simulated setting. These operators ensure the transformations between radiograph and CT to be geometrically consistent, therefore significantly reducing the complexity of learning. We further incorporate the differentiable forward projector into a modified DeepDRR \cite{DBLP:conf/miccai/UnberathZLBFAN18}, which simulates realistic radiographs, to minimize the domain gap between DRRs and real radiographs. 
%3DPN performs reasonably well at generating 3D context on real radiographs, despite intrinsic differences between CT and radiography.
The second stage of XraySyn, called 2D RefineNet (2DRN), further enhances the projected radiograph from its estimated 3D CT. By using a Generative Adversarial Network (GAN) and residual connections, 2DRN produces high quality radiographic views and their respective bone structure. 
In summary, our contributions can be described in four parts:
\begin{enumerate}
    \item We propose a differentiable forward projection operator and incorporate it within a modified DeepDRR, forming a pipeline called CT2Xray that simulates realistic radiographs from CT, propagates gradients, and runs fast.
    \item We propose a 3D PriorNet (3DPN), which incorporates CT2Xray and generates the 3D context from a single radiograph through learning from the paired relationship between simulated radiographs and their CT volumes.
    \item We propose a 2D RefineNet (2DRN), which refines on the 2D radiographs projected from 3DPN's output. By leveraging the availability of CT labels and the CT2Xray pipeline, 2D RefineNet can synthesize not only novel radiograph views, but also the corresponding bone structure.
    \item We examine XraySyn, comprising 3DPN and 2DRN, on real radiographs and find the performance of view synthesis and bone extraction visually accurate, despite the lack of direct supervision in the radiograph domain.
\end{enumerate}



% the network does not need to learn the complex geometric rela



% radiograph simulation algorithm, called CT2Xray, to aid its learning 

% An important piece within XraySyn is a differentiable forward projection algorithm

% The first stage, called 3D PriorNet, or 3DPN, 


 




%(further explain advantage of CT with labels and stuff)


%use a simplified version of DeepDRR[] to produce realistic radiographs. In combination with 


%, and currently there is no way to replicate and incorporate the prior, i.e. the regularity of 3D human anatomy, algorithmically







==> XraySyn New/method.tex <==
\section{Method}
The main goal of this work is to synthesis novel views from a frontal view radiograph, which requires a degree of 3D knowledge. As multi-view dataset is not readily available for real radiographs, our proposed method, XraySyn, composes of two stages. The first stage learns to estimate 3D knowledge under a simulated setting by using CT volumes. The second stage transfers such learning to generate real radiographs. 

The challenge underlying this approach is how to best address the transformation from simulated radiographs to CT volumes, while ensuring the input radiograph can be reproduced from such volume. We first explain the proposed operators that enable learning such a transformation, CT2Xray and Single Image Backprojector. We then introduce XraySyn, which incorporates the two operators for a radiograph-to-CT-to-radiograph algorithm. 



% At the core of our proposed methods is a differentiable forward projection operator and the realistic radiograph simulator \textit{CT2Xray} of which the operator is incorporated in. To our knowledge, CT2Xray is \textit{the first algorithm} that can generate realistic radiographs from CT volumes efficiently with gradient propagation along arbitrary viewpoint. Along with a backprojection operator, which projects radiographs onto 3D space, CT2Xray helps complete the cycle of transformations between radiograph and CT domain. We then introduce XraySyn, which leverages the cycle transformation to learn an end-to-end radiograph-to-CT model under simulated settings, and transfer such a model to real radiographs by finetuning in 2D. 

\begin{figure*}[htb!]
\centering
\includegraphics[width=\textwidth]{XraySyn_net.png}
\caption{The proposed two-stage network structure of XraySyn.
% Haofu: explicitly denote which one is the first stage and which one is the second in the figure.
In the first stage (top), \emph{simulated} radiographs are backprojected (BP) from view $T$, and refined through 3DPN to obtain their CT and bone mask estimates, $V_{\textrm{CT}}$ and $V_{\textrm{mask}}$. Through CT2Xray, $V_{\textrm{CT}}$ and $V_{\textrm{mask}}$ are forward projected (FP) from view $T^{'}$ to calculate the tissue and bone content $t^{\textrm{CT}}_{\textrm{bone}}$ and $t^{\textrm{CT}}_{\textrm{tissue}}$, which are used to simulate the novel view radiograph. In the second stage (bottom), $t^{\textrm{CT}}_{\textrm{bone}}$ and $t^{\textrm{CT}}_{\textrm{tissue}}$ are generated from \emph{real} radiographs through a trained 3DPN, refined through 2DRN, and used to generate the novel view.} %More visualization on CT2Xray is in supplemental material.}
\label{fig:xraysyn_net}
\vspace{-1.5em}
\end{figure*}
% A big challenge in tackling the X-ray view synthesis problem is that real, properly aligned multi-view X-ray images are rare due to the ALARA principle at acquisition; datasets such as CheXpert\cite{DBLP:conf/aaai/IrvinRKYCCMHBSS19} and others provide at most two X-ray views, which are orthogonal to each other and poorly aligned. In this paper, we perform experiments on realistically simulated X-ray images from CT volumes, and prove the effectiveness of our method by applying it on real X-ray images at test time. To this end, we first introduce a realistic and differentiable projection algorithm called CT2Xray in section \ref{sec:ct2xray}, and the view synthesis XraySyn algorithm in section \ref{sec:xraysyn}.
\subsection{CT2Xray}
CT2Xray, as shown in Fig. \ref{fig:xraysyn_net}, has two parts: (i) the differentiable forward projection; (ii) attenuation-based radiograph simulation, which along with the first part forms CT2Xray and transforms a CT volume into a realistic radiograph. To the best of our knowledge, CT2Xray is \textit{the first algorithm} that can generate realistic radiographs from CT volumes with gradient propagation along arbitrary viewpoint.

\textbf{Differentiable forward projector (FP)}.
Let $V_{\textrm{CT}}$ denote a CT image, FP generates a 2D projection of $V_{\textrm{CT}}$ by:
\begin{align} \label{eq:drr}
\begin{aligned}
    I(x) = \textrm{FP}(V_{\textrm{CT}}, T) = \int 
    V_{\textrm{CT}}(T^{-1} p) d\bm{l}(x) \\
     ~\approx \sum_{p \in \bm{l}(x)} V_{\textrm{CT}}(T^{-1} p) \Delta p,
\end{aligned}
\end{align}
where $T$ is a homogeneous matrix that controls the rotation and translation of the view point and $\bm{l}(x)$ is a line segment connecting the simulated x-ray source and detector at $x$. For backpropagation, the gradients of $I$ wrt $V_{\textrm{CT}}$ can be written as
\begin{equation}\label{eq:grad}
 \dfrac{\partial I(x)}{\partial V_{\textrm{CT}}(y)} =
 \begin{cases}
  \Delta p, &\text{if} ~~ Ty \in \bm{l}(x),\\
     0, &\text{otherwise. }
 \end{cases}
\end{equation}
Equations for (\ref{eq:drr}) and (\ref{eq:grad}) can be implemented through massive parallelism with GPUs, where every line integral over the volume is a standalone operation; as such this implementation can be used in online training.

\textbf{CT2Xray}.\label{sec:ct2xray}
Forward projecting CT volumes generates DRRs, which are poor simulations of X-ray images due to the inaccurate assumption that different tissues attenuate the X-ray similarly. DeepDRR \cite{DBLP:conf/miccai/UnberathZLBFAN18} produces a better simulation by avoiding this assumption, but it is not differentiable and hence not amenable for end-to-end learning. We contribute a \textit{differentiable 
X-ray simulation} pipeline, called CT2Xray, which incorporates the differentiable forward projector and produces more realistic radiographs. In~\cite{DBLP:conf/miccai/UnberathZLBFAN18}, a realistic X-ray attenuation $I_{\textrm{atten}}$ is modeled as
\begin{align}
    I_{\textrm{atten}} = \sum_{E}I_{0}e^{-\sum_{m}\mu(m,E)t_{m}} + \textrm{SE} + \textrm{noise},
\end{align}
where $\mu(m,E)$ is the linear attenuation coefficient of material $m$ at energy state $E$ and is measured and known \cite{hubbell1995tables}, $t_{m}$ is the material thickness. $\textrm{SE}$
% Haofu: This term is ambiguous. Is it SxE? then what is S, is SE a function of E? then rewrite it in function way say g(E) where g is the scattering estimation function. Or use some other fonts to distinguish SE from SxE
is the scatter estimation term, $I_{0}$ is the source X-ray intensity. Along with noise, $\textrm{SE}$ and $I_{0}$ are omitted for simplicity.

CT2Xray considers only the bone and tissue materials, that is, $m\in \{\textrm{bone,tissue}\}$. With the aid of a bone mask $V_\textrm{mask}$ and using the differentiable forward projector, it calculates the material thickness wrt the projection parameter $T$ as
\begin{align}
\begin{aligned}
t^{\textrm{CT}}_\textrm{bone}(T)= \textrm{FP}(V_{\textrm{CT}} \odot V_{\textrm{mask}}, T),\\
t^{\textrm{CT}}_\textrm{tissue}(T)= \textrm{FP}(V_{\textrm{CT}} \odot (1-V_{\textrm{mask}}), T).
\end{aligned}
\end{align}
%It separates $V_{\textrm{CT}}$ into two volumes $\{V_\textrm{bone}, V_\textrm{tissue}\}$ by $V_\textrm{bone}= V_{\textrm{CT}} \odot V_{\textrm{mask}}$ and $V_\textrm{tissue}=V_\textrm{CT}-V_\textrm{bone}$, with $V_{\textrm{mask}}$ being the bone mask. The differentiable forward projector is then used to calculate $t^{\textrm{CT}}_m =\textrm{FP}(V_{m}, T)$. $t^{\textrm{CT}}_{\textrm{bone}}(T)$ and $t^{\textrm{CT}}_{\textrm{tissue}}(T)$ from the respective volumes, as shown in Fig. \ref{fig:xraysyn_net}. 
Radiographs are typically stored and viewed as inverted versions of the measured attenuation; therefore, CT2Xray can be expressed as
\begin{align}\label{eq:ct2xray}
    \textrm{CT2Xray}(V_{\textrm{CT}}, V_{\textrm{mask}}, T) = \textrm{max}(I^{T}_{\textrm{atten}}) - I^{T}_{\textrm{atten}},
\end{align}
with
\begin{equation}\label{eq:ct2xray_eq}
I^{T}_{\textrm{atten}} = \sum_{E}e^{-\sum_{m}\mu(m, E)t^{\textrm{CT}}_{m}(T)}.
\end{equation}

%(move below to implementation detail or supplemental material?)
% Compared to DeepDRR, we discard the calculations of air attenuation, scatter estimation, noise injection, and reduce the considered energy states from 151 to 10 states. We find that such simplification leads better contrast on the simulated radiographs for our dataset, and makes CT2Xray more efficient for online training.


%, thus making the calculation of $I_{atten}$ differentiable. 
%  CT2Xray discards the calculations of air attenuation, scatter estimation, and noise injection, which are modelled in DeepDRR for physical accuracy. We find that these calculations can lead to noise-like patterns, reduction in contrast, or lack in robustness. By removing these calculations, we make CT2Xray fast enough to be used for online training and end-to-end differentiable. Furthermore, as the tissue volume is a combination of many materials, $\mu(tissue, E)$ may inaccurately represent the attenuation coefficients of all tissues. Further separating tissue material is an intractable problem, thus we introduce a weight coefficient $\omega_{tissue}$ for $\mu(tissue, E)$ to modulate the relative contribution of bone and tissue attenuation to the final output, and provide an extra degree of freedom. As shown in Fig. \ref{fig:projector}, the output of CT2Xray is much more realistic than traditional DRR images. For more details on the implementation of CT2Xray, please refer to the supplemental material section.


\textbf{Single image backprojector (BP)}.
While CT2Xray generates radiographs from CT volumes, an inverse function is needed to transform radiographs back to the respective CT volumes. Such a transformation is clearly ill-posed; however, we can formulate an inverse function of the forward projector to properly place the input X-ray image in 3D. We call such an inverse function the \textit{single image backprojector}. Following a similar formulation from general backprojection algorithm, which reconstructs CBCT from multi-view radiographs as described in \cite{KINAHAN2004421}, the single image backprojector (BP) is expressed as the following:
\begin{equation} \label{eq:bp}
 V^{T}_{\textrm{BP}}(y) = \textrm{BP}(I(x), T) = 
 \begin{cases}
   \frac{I(x)}{\lvert \bm{l}(x) \rvert \Delta p}, &\text{if} ~~ Ty \in \bm{l}(x),\\
     0, &\text{otherwise. }
 \end{cases}
\end{equation}
By substituting $V^{T}_{\textrm{BP}}$ in (\ref{eq:bp}) into $V_{\textrm{CT}}$ in (\ref{eq:drr}), the same $I$ is recovered under view $T$, hence we denote $V^{T}_{\textrm{BP}}$ obtained in this way as the backprojection of $I$ at view $T$. While the same image-wise consistency does not generally apply to CT2Xray, i.e., substituting (\ref{eq:bp}) into (\ref{eq:ct2xray}) does not recover $I$. We show that by using a CNN to complement the single image backprojector, such consistency can be better approximated due to geometric consistency.

\subsection{XraySyn}
% \begin{figure*}[htb]
% \centering
% \includegraphics[width=\textwidth]{imgs/XraySyn_net_new.png}
% \caption{The proposed network structure of XraySyn and XraySyn+. XraySyn is shown in the grey area, which incorporates our proposed CT2Xray and single image backprojection operators to assist the geometric transformation between the X-ray and CT domain. XraySyn+ further incorporates XraySyn by projecting the estimated volume $V_{XS}$ onto a manifold discovered by a pre-trained 3D PGGAN on chest CTs to obtain a more detailed $V_{XS+}$.}
% \label{fig:network}
% \end{figure*}
XraySyn is trained in two stages, as shown in Fig. \ref{fig:xraysyn_net}. The simulation stage trains a radiograph-to-CT transformation network, called 3D PriorNet, and with help of CT2Xray generate radiographic views from the estimated CT. The real-radiograph stage, which trains a 2D RefineNet, then further closes the domain gap between simulated and real radiographs. Due to the need for calculating the material-dependent attenuation, we also gain the ability to transfer labels from the CT domain to the radiograph domain, in our case with CT bone labels, and achieve bone extraction on real radiographs. 

\textbf{3D PriorNet (3DPN)}.
Under simulated setting, Single Image Backprojector produces $V^{T}_{\textrm{BP}}$ from input view radiograph $I^{T}$, and CT2Xray produces a desired view radiograph $I^{T^{'}}$ from $V_{\textrm{CT}}$ and $V_{\textrm{mask}}$; to complete the end-to-end radiograph-to-CT generation, a function $G$ is needed to recover $V_{\textrm{CT}}$ and $V_{\textrm{mask}}$ from $V^{T}_{\textrm{BP}}$. Mathematically, the generation process between radiograph and CT can be expressed as:
\begin{equation} \label{eq:xraysyn}
\begin{aligned}
    \{V_{\textrm{CT}}, V_{\textrm{mask}}\} = G(\textrm{BP}(I^{T}_{in}, T); \theta), \\ I^{T^{'}}_{\textrm{CT}} = \textrm{CT2Xray}(V_{\textrm{CT}}, V_{\textrm{mask}},T^{'}),
\end{aligned}
\end{equation}
where $\theta$ represents the parameters in $G$. We use a 3D UNet \cite{DBLP:conf/miccai/CicekALBR16} structure for $G$. The loss functions for training $G$ need to ensure consistency both in CT and radiograph domains, and are defined as:
%Leveraging the geometrically consistent translation between the 2D and 3D domains, the losses for training $G$ are defined as:
\begin{align}\label{eqn:loss3dpn}
    \mathcal{L}_{G} &= \lambda_{\textrm{CT}}\mathcal{L}_{\textrm{CT}} + \lambda_{\textrm{mask}}\mathcal{L}_{\textrm{mask}} +  \lambda_{\textrm{xray}}(\mathcal{L}^{T}_{\textrm{xray}}+\mathcal{L}^{T^{'}}_{\textrm{xray}}), 
\end{align}
where $\lambda_{\textrm{CT}}$, $\lambda_{\textrm{mask}}$, and $\lambda^{T}_{\textrm{xray}}$ are weights; $\mathcal{L}_{\textrm{CT}}$, $\mathcal{L}_{\textrm{mask}}$, and $\mathcal{L}^{T}_{\textrm{xray}}$ are defined as:
\begin{align}\label{eqn:loss3dpn_2}
\begin{aligned}
\mathcal{L}_{\textrm{CT}} = \lVert V_{\textrm{CT}} - V_{\textrm{gt}} \rVert_1, ~~
\mathcal{L}_{\textrm{mask}} = \textrm{CE}(V_{\textrm{mask}}, V^{\textrm{gt}}_{\textrm{mask}}),\\
\mathcal{L}^{T}_{\textrm{xray}}=\lVert I^{T}_{\textrm{CT}} - I^{T}_{\textrm{in}} \rVert_1 + \sum_{m}\lVert t^{\textrm{CT}}_{\textrm{m}}(T) - t^{\textrm{gt}}_{\textrm{m}}(T) \rVert_1,
\end{aligned}
\end{align}
where CE refers to the cross entropy loss and  $\mathcal{L}^{T^{'}}_{\textrm{xray}}$ is defined similarly as $\mathcal{L}^{T}_{\textrm{xray}}$.
%It is worth noting that 

% The LSGAN loss for training XraySyn is defined as:
% \begin{align*}
% \mathcal{L}_{LSGAN}(D)=\mathbb{E}(D(V_{CT})-1)^2 + \mathbb{E}(D(V_{XS})-0)^2\\
% \mathcal{L}_{LSGAN}(G)=\mathbb{E}(D(V_{XS})-1)^2,
% \end{align*}
% where $D$ is a 3D discriminator network.% for more network details please refer to Supplemental Material.

\textbf{2D RefineNet (2DRN)}. While 3DPN $\textrm{G}$ estimates a degree of 3D context from a radiograph, such estimation is both coarse in quality, due to the ill-posed nature, and in resolution, due to memory constraint.
%The further the novel view angle $T^{'}$ is away from the input view angle $T$, the more variations become possible for the novel view radiographs $I^{T^{'}}_{CT}$. As 3DPN is optimized for L1 consistency, $I^{T^{'}}_{CT}$ takes the expectation across all the variations, which leads loss in detail.
Furthermore, there exists a domain gap between real and simulated radiograph. To address these issues, a second stage, called 2DRN, is introduced. 2DRN has two goals: (i) to generate realistic radiographs from the output of 3DPN with higher resolution, and (ii) to do so with small refinements on $t^{\textrm{CT}}_{m}$ such that we can still obtain the material decomposition of the output radiograph. Conceptually, 2DRN can be understood as a part of an augmented, learnable CT2Xray. 2DRN is constructed in two parts. The main refinement network $\mathcal{F}$ is based on Residual Dense Network (RDN) \cite{DBLP:conf/cvpr/ZhangTKZ018}; additionally, a fully convolutional network $\mathcal{M}$ is used to generate certain convolutional layer parameters in $\mathcal{F}$ directly from the input $I^{T}_{\textrm{in}}$. The purpose of $\mathcal{M}$ is to shuffle high level information that may be lost during the process of 3DPN. Overall, the refinement on $t^{\textrm{CT}}_{m}$ is expressed as:
\begin{align}\label{eqn:loss2drn}
    t^{\textrm{ref}}_{m}(T) =t^{\textrm{CT}}_{m}(T)+ \mathcal{F}(t^{\textrm{CT}}_{m};\phi, 
    \mathcal{M}(I^{T}_{\textrm{in}})), 
\end{align}
where $\phi$ and $\mathcal{M}(I^{T}_{\textrm{in}})$ represent the parameters in $\mathcal{F}$. Replacing $t^{\textrm{CT}}_{m}$ in (\ref{eq:ct2xray}) with $t^{\textrm{ref}}_{m}$ yields an augmented CT2Xray:
\begin{align}\label{eq:ct2xray_aug}
\begin{aligned}
    \textrm{CT2Xray}_{\textrm{aug}}(V_{\textrm{CT}}, V_{\textrm{mask}}, T) = \textrm{max}(I^{T}_{\textrm{ref}}) - I^{T}_{\textrm{ref}},
\end{aligned}
\end{align}
where $I^{T}_{\textrm{ref}} = \sum_{E}e^{-\sum_{m}\mu(m, E)t^{ref}_{m}}$. 
Similarly, the final view synthesis results are defined as $I^{T^{'}}_{\textrm{final}} = \textrm{CT2Xray}_{\textrm{aug}}(V_{\textrm{CT}}, V_{\textrm{mask}},T^{'})$.
A Least-Square GAN (LSGAN) is used to ensure $I^{T^{'}}_{\textrm{final}}$ is statistically similar to $I^{T}_{\textrm{in}}$ when $T^{'}$ and $T$ are relatively close. The overall loss function for 2DRN is described as:
\begin{align}\label{eqn:loss2drn_2}
\mathcal{L}_{\textrm{2DRN}}=\lambda_{\textrm{recon}}\lVert I^{T}_{\textrm{final}} - I^{T}_{\textrm{in}} \rVert_1 + \lambda_{\textrm{GAN}}\mathcal{L}_{\textrm{LSGAN}}(I^{T^{'}}_{\textrm{final}}, I^{T}_{\textrm{in}}).
\end{align}
$\mathcal{L}_{\textrm{LSGAN}}$ is defined as:
\begin{align}\label{eqn:lossGAN}
\begin{aligned}
\mathcal{L}^{\mathcal{D}}_{\textrm{LSGAN}}(I^{T^{'}}_{\textrm{final}}, I^{T}_{\textrm{in}})=\mathbb{E}(\mathcal{D}(I^{T}_{\textrm{im}}-1)^2)) + \mathbb{E}(\mathcal{D}(I^{T^{'}}_{\textrm{final}}-0)^2),\\
\mathcal{L}^{\mathcal{G}}_{\textrm{LSGAN}}(I^{T^{'}}_{\textrm{final}})=\mathbb{E}(\mathcal{D}(I^{T^{'}}_{\textrm{final}}-1)^2),
\end{aligned}
\end{align}
where $\mathcal{G}$ indicates generator, in this case the composition of $G$, $\mathcal{F}$, and $\mathcal{M}$. $\mathcal{D}$ indicates the discriminator. 
% less precise the 3DPN-synthesized novel view radiographs become. This is to be expected, as possible variation for novel view radiographs is large and 

% 1. the ill-posed nature of 2D-to-3D inversion, and 2. the domain gap between real and simulated radiographs. Naturally, an additional 

% As our goal is to synthesize novel view radiographs, 




% \textbf{XraySyn+}. 
% Recovering a $V_{CT}$ with anatomically realistic details from $V^{T}_{BP}$ is very difficult
% due to the challenging nature in 2D-to-3D inversion. The conditional GAN setup as described in Eq. \ref{eqn:loss}, when dominated by the pixel and voxel-wise losses, inhibit the ability of GAN to generate fine and realistic details. Unfortunately, anatomical details like bones are disproportionally presented in X-ray images compared to their volume size due to their high material density and attenuation rate, and an incomplete recovery of such details leads to unrealistic X-ray images.

% In order to enhance XraySyn's ability in generating complete and realistic anatomic details, we propose an alternative version of XraySyn called XraySyn+. XraySyn+ leverages recent advances in unconditional GANs, specifically with PGGAN, which are able to produce very realistic images. We first training a 3D variant of PGGAN that can generate CT volumes. A 3D encoder $F$ is then introduced to project $V_{XS}$ onto the manifold spanned by the PGGAN. The resulting X-ray projections and CT volumes are described as:
% \begin{align*}
% V_{XS+} = PGGAN(F(V_{XS}; \phi); \psi)\\
% I^{T^{'}}_{XS+} = CT2Xray(V_{XS+},T^{'}),
% \end{align*}
% where $\phi$ and $\psi$ are parameters for $F$ and the PGGAN, respectively. The losses for training $F$ is defined as:
% \begin{align}\label{eqn:loss+}
%     \mathcal{L}_{F} &= \lambda_{CT}\mathcal{L}^{F}_{CT} + \lambda_{xray}\mathcal{L}^{F}_{xray} + \lambda_{code}\mathcal{L}_{code},
% \end{align}
% where $\mathcal{L}^{F}_{CT}$ and $\mathcal{L}^{F}_{xray}$ are as similarly defined in (\ref{eqn:loss2}) using $V^{T}_{XS+}$ and $I^{T^{'}}_{XS+}$. A code consistency loss $\mathcal{L}_{code}$ is introduced to encourage the projections of $V_{XS}$ and the groundtruth CT volume to be similar. It is defined as:
% \begin{align}\label{eqn:code_consis}
%     \mathcal{L}_{code} &= \lVert F(V_{XS+}; \phi) - F(V_{CT}; \phi) \rVert_2
% \end{align}
% Lastly, similar to the hybrid method described by Zhu et al. \cite{DBLP:conf/eccv/ZhuKSE16}, the latent code $z_{Recon}$ is updated for 1000 steps for each individual volume by the solving for the following optimization problem:
% \begin{align}\label{eqn:optim}
%     \argmin_{z} \lVert CT2Xray(PGGAN(z), T) - I^{T}_{in} \rVert_1,
% \end{align}
% where $z$ is initialized with $F(V_{XS+}; \phi)$. 


%Similar to the forward projector, the single image backprojector can be run at real time through the use of GPU.
%Further note that this is unlike the filtered backprojection algorithm commonly used in CT reconstruction, as only a single image is used.

%TODO: add the 3D UNet part using the above formulations.




%As $\mu(m, E)$ is a scalar value measured by \cite{hubbell1995tables}, The main challenge to making the entire pipeline differentiable is the calculations of $t(m)$. 




% As shown in Fig. \ref{fig:projector}, the algorithm first separates the lung CT $V_{CT}$ into a bone and tissue volume, $V_{bone}$ and $V_{tissue}$, to allow attenuation calculation of different materials. This step can be performed manually, through a dedicated segmentation algorithm, or Housefield Unit(HU) thresholding. Forward projection is performed individually over $V_{bone}$ and $V_{tissue}$ to obtain $I_{bone}$ and $I_{tissue}$, which represents the thickness of the material during every path. The attenuation rates of $I_{bone}$ and $I_{tissue}$ are calculated over a spectrum of 151 energy states\cite{hubbell1995tables}, where higher energy leads to less attenuation. The weighted sum of bone and tissue attenuation $\mu_{bone}$ and $\mu_{tissue}$ goes through the exponential decay model described as

% \begin{align}
%     I_{atten}^{i} = e^{\mu_{bone}^{i} + \omega_{tissue} \times \mu_{tissue}^{i}}, I_{Xray}^{'} = \sum_{i} I_{atten}^{i}
% \end{align}

% where $i$ represents the different energy state, and $I_{Xray}^{'}$ represents the X-ray image in terms of attenuation rate. In addition to calculating gradients for the entire pipeline to enable end-to-end training, CT2Xray discards the calculation of air attenuation, scatter estimation, and noise injection in DeepDRR to reduce the computation costs. While these processes realistically model the X-ray imaging physics, we find that they minimally affect the image quality. Furthermore, as $V_{tissue}$ is a combination of many materials, we find that $\mu_{tissue}$ may inaccurately represent the attenuation contribution of tissues. Since further separating tissue material is an intractable problem, we introduce a weight parameter $\omega_{tissue}$ to modulate between the relative contribution of bone and tissue attenuation to the final output. Lastly, clinical X-ray images are printed as inverted versions of $I_{Xray}^{'}$ and oftentimes clipped into certain dynamic range for better regional contrast; this process is also simulated in CT2Xray as the last stage in Fig. \ref{fig:projector}, and can be described as:
% \begin{align}
%     I_{Xray} = Clip(max(I_{Xray}^{'}) - I_{Xray}^{'}, floor, ceiling),
% \end{align}
% where the floor and ceiling values depends on the intended dynamic range.





==> XraySyn New/method_backup.tex <==
\section{Method}
At the core of our proposed methods is a differentiable forward projector called the \textit{CT2Xray} operator. To our best knowledge, the CT2Xray operator is \textit{the first algorithm} that can generate realistic X-ray images from a CT volume in a \textit{differentiable} and \textit{fast} fashion along arbitrary viewpoint. Combined with the backprojection operator, which projects X-ray images onto 3D space, these two operators help complete the cycle of transformation between the X-ray and CT domain. We then introduce XraySyn, which leverages the cycle transformation to train an end-to-end X-ray view synthesis model, and XraySyn+, which addresses the challenges in generating realistic anatomic structures.
\begin{figure*}[htb]
\centering
\includegraphics[width=\textwidth]{XraySyn_net.png}
\caption{The differentiable CT2Xray projection algorithm. CT2Xray is differentiable, fast enough to be used for online training, and generates highly realistic X-ray simulations.}
\label{fig:projector}
\end{figure*}
% A big challenge in tackling the X-ray view synthesis problem is that real, properly aligned multi-view X-ray images are rare due to the ALARA principle at acquisition; datasets such as CheXpert\cite{DBLP:conf/aaai/IrvinRKYCCMHBSS19} and others provide at most two X-ray views, which are orthogonal to each other and poorly aligned. In this paper, we perform experiments on realistically simulated X-ray images from CT volumes, and prove the effectiveness of our method by applying it on real X-ray images at test time. To this end, we first introduce a realistic and differentiable projection algorithm called CT2Xray in section \ref{sec:ct2xray}, and the view synthesis XraySyn algorithm in section \ref{sec:xraysyn}.
\subsection{CT2Xray operator}
The CT2Xray operator is explained in two parts: (i) the core differentiable forward projection algorithm; (ii) the X-ray simulation algorithm, which along with the first part forms the CT2Xray operator that directly transforms a CT volume into realistic X-ray simulations.


\textbf{Differentiable Forward Projector}.
Let $V_{CT}$ denote a CT image, the forward projector generates a 2D projection of $V_{CT}$ by:
\begin{align} \label{eq:drr}
\begin{aligned}
    I(x) = FP(V_{CT}) = \int 
    V_{CT}(T^{-1} p) d\bm{l}(x) \\
     ~\approx \sum_{p \in \bm{l}(x)} V_{CT}(T^{-1} p) \Delta p
\end{aligned}
\end{align}
where $T$ is a homogeneous matrix that controls the rotation and translation of the view point and $\bm{l}(x)$ is a line segment connecting the simulated x-ray source and detector at $x$. For backpropagation, the gradients of $I$ with respect to $V_{CT}$ can be written as
\begin{equation}\label{eq:grad}
 \dfrac{\partial I(x)}{\partial V_{CT}(y)} =
 \begin{cases}
  \Delta p, &\text{if} ~~ Ty \in \bm{l}(x),\\
     0, &\text{otherwise. }
 \end{cases}
\end{equation}
Calculations for (\ref{eq:drr}) and (\ref{eq:grad}) can be done through massive parallelism with GPUs, where every line integral over the volume is standalone%a standalone process
; as such this implementation can be used in online training.

\textbf{CT2Xray}.\label{sec:ct2xray}
Forward projecting on CT volumes generates DRRs, which are poor simulations of X-ray images due to the inaccurate assumptions. Inspired by DeepDRR \cite{DBLP:conf/miccai/UnberathZLBFAN18}, we incorporate the differentiable forward projector into a more realistic X-ray simulation pipeline, called CT2Xray. Unberath et al. proposes that a realistic X-ray attenuation $I_{atten}$ can be modeled as
\begin{align}
    I_{atten} = \sum_{E}I_{0}e^{-\sum_{m}\mu(m, E)t(m)} + SE + noise,
\end{align}
where $\mu(m, E)$ is the linear attenuation coefficient of material $m$ at energy state $E$, $t(m)$ is the material thickness, $SE$ is the estimation term that models X-ray scattering, and $I_{0}$ is the source X-ray intensity. For simplicity, $I_{0}$ is considered at the unit intensity. By first separating $V_{CT}$ into different materials $V_{m}$, our differentiable forward projector can be used to calculate $t(m)$, where $t(m) = FP(V_{m})$. %, thus making the calculation of $I_{atten}$ differentiable. 
 CT2Xray discards the calculations of air attenuation, scatter estimation, and noise injection, which are modelled in DeepDRR for physical accuracy. We find that these calculations can lead to noise-like patterns, reduction in contrast, or lack in robustness. By removing these calculations, we make CT2Xray fast enough to be used for online training and end-to-end differentiable. Furthermore, as the tissue volume is a combination of many materials, $\mu(tissue, E)$ may inaccurately represent the attenuation coefficients of all tissues. Further separating tissue material is an intractable problem, thus we introduce a weight coefficient $\omega_{tissue}$ for $\mu(tissue, E)$ to modulate the relative contribution of bone and tissue attenuation to the final output, and provide an extra degree of freedom. As shown in Fig. \ref{fig:projector}, the output of CT2Xray is much more realistic than traditional DRR images. For more details on the implementation of CT2Xray, please refer to the supplemental material section.


\textbf{Single X-ray Backprojector}.
While CT2Xray enables a transformation from a CT volume to an X-ray image, an inverse function for CT2Xray is needed to transform a single X-ray image to a CT volume. Such a 2D-to-3D transformation is clearly ill-posed; however, we can formulate an inverse function of the forward projector to properly place the input X-ray image in 3D and ease the challenge in recovering the same X-ray image through a data-driven way. We name such an inverse function the \textit{single X-ray backprojector}. Following the formulation of general 3D backprojection algorithm for many X-ray images, e.g. as described in \cite{KINAHAN2004421}, we use a simplified version for single X-ray backprojector, where
\begin{equation} \label{eq:bp}
 V^{T}_{BP}(y) = BP(I(x)) = 
 \begin{cases}
   \frac{I(x)}{\lvert \bm{l}(x) \rvert \Delta p}, &\text{if} ~~ Ty \in \bm{l}(x),\\
     0, &\text{otherwise. }
 \end{cases}
\end{equation}
By substituting $V^{T}_{BP}$ in (\ref{eq:bp}) into $V_{CT}$ in (\ref{eq:drr}), the same $I$ is recovered under view $T$, hence we denote $V^{T}_{BP}$ obtained in this way as the backprojection of $I$ at view $T$. While the same image-wise consistency does not generally apply to CT2Xray, we show that by adding a CNN to complement the single X-ray backprojector, such consistency can be well approximated due to geometric consistency.

\subsection{XraySyn}
\begin{figure*}[htb]
\centering
\includegraphics[width=\textwidth]{imgs/XraySyn_net_new.png}
\caption{The proposed network structure of XraySyn and XraySyn+. XraySyn is shown in the grey area, which incorporates our proposed CT2Xray and single image backprojection operators to assist the geometric transformation between the X-ray and CT domain. XraySyn+ further incorporates XraySyn by projecting the estimated volume $V_{XS}$ onto a manifold discovered by a pre-trained 3D PGGAN on chest CTs to obtain a more detailed $V_{XS+}$.}
\label{fig:network}
\end{figure*}

The single X-ray backprojector produces a $V^{T}_{BP}$ from the input X-ray view $I^{T}$, and CT2Xray produces an output X-ray view $I^{T^{'}}$ from $V_{CT}$; to complete the end-to-end X-ray view synthesis process, a function $G$ is needed to recover $V_{CT}$ from $V^{T}_{BP}$. Mathematically, the overall view synthesis process can be expressed as:
\begin{equation} \label{eq:xraysyn}
    V_{XS} = G(BP(I^{T}_{in}, T); \theta), ~~ I^{T^{'}}_{XS} = CT2Xray(V_{XS},T^{'}),
\end{equation}
where $\theta$ represents the parameters in the CNN-based function $G$. %As a 2D UNet structure is often used in image-to-image tasks, e.g. pix2pix, 
We use a 3D UNet \cite{DBLP:conf/miccai/CicekALBR16} to construct $G$. Leveraging the geometrically consistent translation between the 2D and 3D domains, the losses for training $G$ are defined as:
\begin{align}\label{eqn:loss}
    \mathcal{L}_{G} &= \lambda_{CT}\mathcal{L}^{G}_{CT} + \lambda_{xray}\mathcal{L}^{G}_{xray} + \lambda_{GAN}\mathcal{L}_{LSGAN}, 
\end{align}
where $\lambda_{CT}$, $\lambda_{xray}$, and $\lambda_{GANs}$ are weights for different losses. $\mathcal{L}^{G}_{CT}$ and $\mathcal{L}^{G}_{xray}$ are defined as:
\begin{align}\label{eqn:loss2}
\mathcal{L}^{G}_{xray}=\lambda_{in}\lVert I^{T}_{XS} - I^{T}_{in} \rVert_1 + \lambda_{new}\lVert I^{T^{'}}_{XS} - I^{T^{'}}_{gt} \rVert_1 \\
\mathcal{L}^{G}_{CT} = \lVert V_{XS} - V_{CT} \rVert_1, 
\end{align}
where $\lambda_{in}$ and $\lambda_{new}$ are perspective weights for the input X-ray view and the new X-ray view. The LSGAN loss for training XraySyn is defined as:
\begin{align*}
\mathcal{L}_{LSGAN}(D)=\mathbb{E}(D(V_{CT})-1)^2 + \mathbb{E}(D(V_{XS})-0)^2\\
\mathcal{L}_{LSGAN}(G)=\mathbb{E}(D(V_{XS})-1)^2,
\end{align*}
where $D$ is a 3D discriminator network.% for more network details please refer to Supplemental Material.


\textbf{XraySyn+}. 
Recovering a $V_{CT}$ with anatomically realistic details from $V^{T}_{BP}$ is very difficult
due to the challenging nature in 2D-to-3D inversion. The conditional GAN setup as described in Eq. \ref{eqn:loss}, when dominated by the pixel and voxel-wise losses, inhibit the ability of GAN to generate fine and realistic details. Unfortunately, anatomical details like bones are disproportionally presented in X-ray images compared to their volume size due to their high material density and attenuation rate, and an incomplete recovery of such details leads to unrealistic X-ray images.

In order to enhance XraySyn's ability in generating complete and realistic anatomic details, we propose an alternative version of XraySyn called XraySyn+. XraySyn+ leverages recent advances in unconditional GANs, specifically with PGGAN, which are able to produce very realistic images. We first training a 3D variant of PGGAN that can generate CT volumes. A 3D encoder $F$ is then introduced to project $V_{XS}$ onto the manifold spanned by the PGGAN. The resulting X-ray projections and CT volumes are described as:
\begin{align*}
V_{XS+} = PGGAN(F(V_{XS}; \phi); \psi)\\
I^{T^{'}}_{XS+} = CT2Xray(V_{XS+},T^{'}),
\end{align*}
where $\phi$ and $\psi$ are parameters for $F$ and the PGGAN, respectively. The losses for training $F$ is defined as:
\begin{align}\label{eqn:loss+}
    \mathcal{L}_{F} &= \lambda_{CT}\mathcal{L}^{F}_{CT} + \lambda_{xray}\mathcal{L}^{F}_{xray} + \lambda_{code}\mathcal{L}_{code},
\end{align}
where $\mathcal{L}^{F}_{CT}$ and $\mathcal{L}^{F}_{xray}$ are as similarly defined in (\ref{eqn:loss2}) using $V^{T}_{XS+}$ and $I^{T^{'}}_{XS+}$. A code consistency loss $\mathcal{L}_{code}$ is introduced to encourage the projections of $V_{XS}$ and the groundtruth CT volume to be similar. It is defined as:
\begin{align}\label{eqn:code_consis}
    \mathcal{L}_{code} &= \lVert F(V_{XS+}; \phi) - F(V_{CT}; \phi) \rVert_2
\end{align}
Lastly, similar to the hybrid method described by Zhu et al. \cite{DBLP:conf/eccv/ZhuKSE16}, the latent code $z_{Recon}$ is updated for 1000 steps for each individual volume by the solving for the following optimization problem:
\begin{align}\label{eqn:optim}
    \argmin_{z} \lVert CT2Xray(PGGAN(z), T) - I^{T}_{in} \rVert_1,
\end{align}
where $z$ is initialized with $F(V_{XS+}; \phi)$. 


%Similar to the forward projector, the single image backprojector can be run at real time through the use of GPU.
%Further note that this is unlike the filtered backprojection algorithm commonly used in CT reconstruction, as only a single image is used.

%TODO: add the 3D UNet part using the above formulations.




%As $\mu(m, E)$ is a scalar value measured by \cite{hubbell1995tables}, The main challenge to making the entire pipeline differentiable is the calculations of $t(m)$. 




% As shown in Fig. \ref{fig:projector}, the algorithm first separates the lung CT $V_{CT}$ into a bone and tissue volume, $V_{bone}$ and $V_{tissue}$, to allow attenuation calculation of different materials. This step can be performed manually, through a dedicated segmentation algorithm, or Housefield Unit(HU) thresholding. Forward projection is performed individually over $V_{bone}$ and $V_{tissue}$ to obtain $I_{bone}$ and $I_{tissue}$, which represents the thickness of the material during every path. The attenuation rates of $I_{bone}$ and $I_{tissue}$ are calculated over a spectrum of 151 energy states\cite{hubbell1995tables}, where higher energy leads to less attenuation. The weighted sum of bone and tissue attenuation $\mu_{bone}$ and $\mu_{tissue}$ goes through the exponential decay model described as

% \begin{align}
%     I_{atten}^{i} = e^{\mu_{bone}^{i} + \omega_{tissue} \times \mu_{tissue}^{i}}, I_{Xray}^{'} = \sum_{i} I_{atten}^{i}
% \end{align}

% where $i$ represents the different energy state, and $I_{Xray}^{'}$ represents the X-ray image in terms of attenuation rate. In addition to calculating gradients for the entire pipeline to enable end-to-end training, CT2Xray discards the calculation of air attenuation, scatter estimation, and noise injection in DeepDRR to reduce the computation costs. While these processes realistically model the X-ray imaging physics, we find that they minimally affect the image quality. Furthermore, as $V_{tissue}$ is a combination of many materials, we find that $\mu_{tissue}$ may inaccurately represent the attenuation contribution of tissues. Since further separating tissue material is an intractable problem, we introduce a weight parameter $\omega_{tissue}$ to modulate between the relative contribution of bone and tissue attenuation to the final output. Lastly, clinical X-ray images are printed as inverted versions of $I_{Xray}^{'}$ and oftentimes clipped into certain dynamic range for better regional contrast; this process is also simulated in CT2Xray as the last stage in Fig. \ref{fig:projector}, and can be described as:
% \begin{align}
%     I_{Xray} = Clip(max(I_{Xray}^{'}) - I_{Xray}^{'}, floor, ceiling),
% \end{align}
% where the floor and ceiling values depends on the intended dynamic range.





==> XraySyn New/related_work.tex <==
\section{Related work}

\subsubsection{View synthesis from a single image }

There is a long history of research in natural image view synthesis. For relevancy and brevity, we focus on recent advances in view synthesis based on a single image and with the use of CNN. One approach to tackling such a task is to generate the new view in an image-to-image fashion. Some methods \cite{DBLP:conf/nips/ChenCDHSSA16,DBLP:conf/nips/KulkarniWKT15} propose to generate a disentangled space where the image can be projected to and modified from to synthesize new views, while others \cite{DBLP:conf/cvpr/ParkYYCB17,DBLP:conf/eccv/SunHLZL18,DBLP:conf/eccv/TatarchenkoDB16,DBLP:conf/eccv/ZhouTSME16} rely on GANs to generate the information that is occluded from the original view. In general, the image-to-image approach is based on sufficient pixel correspondence between views, which provide understanding for recovery in either the image space or latent space. Such pixel correspondence is much weaker between X-ray views. In spirit, our method is more similar to the 3D shape generation approaches \cite{DBLP:conf/eccv/GirdharFRG16,DBLP:conf/eccv/ChoyXGCS16,DBLP:journals/corr/abs-1911-13225,DBLP:conf/nips/XuWCMN19,DBLP:conf/iccv/Gkioxari0M19,DBLP:journals/corr/abs-1802-05384} that concern the generation of 3D surfaces, which are less ill-posed than generating 3D volumes. 

\subsubsection{Radiograph simulation and transformation to CT}
Due to the lack of multi-view radiographs and the difficulties in correctly labelling them, data-driven methods that require large number of radiographs often turn to CT-based radiograph simulations. While Monte-Carlo (MC) methods based on imaging physics \cite{badal2009accelerating,sisniega2013monte,schneider2000correlation} can lead to highly realistic radiograph simulations, they are time-consuming and not scalable. Many works \cite{li2020high,DBLP:conf/miccai/GozesG18,DBLP:conf/cvpr/YingGMWWZ19,DBLP:conf/miccai/AlbarqouniFN17,8363572} use DRRs, which are less realistic but computationally inexpensive radiograph simulations, to perform tasks such as bone enhancement, bone suppression, disease identification, CT reconstruction, etc. In particular, Ying \cite{DBLP:conf/cvpr/YingGMWWZ19} addresses the discrepancy between DRRs and real radiographs by training an additional domain adaptation network. Henzler \cite{DBLP:journals/cgf/HenzlerRRR18} uses real cranial X-ray images acquired in a controlled setting to recover the 3D bone structure. As clinical evidence supports that bone suppression on radiograph can improve diagnostic accuracy \cite{laskey1996dual}, Li \cite{li2020high} proposes to achieve bone suppression by learning a bone segmentation network based on DRRs, and apply the network on real radiographs with handcrafted post-processes. Recently, DeepDRR \cite{DBLP:conf/miccai/UnberathZLBFAN18} is proposed to model DRR generation more accurately by replicating similar procedures from the MC simulation counterpart, and shows that CNN models trained on such simulations are able to generalize better on real radiographs. 



==> XraySyn New/supplemental_material.tex <==
\appendix

% \input{imgs/supplemental/versus}
\begin{figure*}[]
\centering
\includegraphics[width=\textwidth]{imgs/ct2xray_vis.png}
\caption{A visualization of the CT2Xray component within XraySyn.}
\label{fig:ct2xray_vis}
\end{figure*}
\section{Network architecture}

The proposed XraySyn consists of 3D PriorNet (3DPN) and 2D RefineNet (2DRN). The general model architectures of 3DPN and 2DRN follow 3D-UNet \cite{DBLP:conf/miccai/CicekALBR16} and RDN \cite{DBLP:conf/cvpr/ZhangTKZ018}. For 3DPN, the exact network structure is presented in Table \ref{table:3DPN-fg}. For 2DRN, we use RDN with sixteen Residual Dense Blocks (RDBs), eight convolutional layers per RDB, and growth rate of sixty-four. After the Global Feature Fusion (GFF) layer, an additional convolutional layer with kernel size of one is introduced where the filter parameters are generated by a subnetwork $\mathcal{M}$. The upsampling layers then upsample spatial dimensions from $128 \times 128$ to $256 \times 256$, the output channel dimension is two, for bone and tissue. The exact network structure of $\mathcal{M}$ is presented in Table \ref{table:2DRN-M-fg} and is a fully convolutional network. As the spatial dimension decreases four times at every convolutional layer with a stride of two, $\mathcal{M}$ is computationally efficient both in memory and speed. In the network tables, $N_c$ denotes the number of output channels, $C'$ denotes the channel dimension of generated features $F^{LR}$. We use `K\#-C\#-S\#-P\#' to denote the configuration of the convolution layers, where `K', `C', `S' and `P' stand for the kernel, input channel, stride and padding size, respectively. 
\input{imgs/supplemental/network_M}
\input{imgs/supplemental/network_3DPN}

2D Refiner as described in Ablation study also uses the RDN structure for refinement on $\textrm{FP}(\textrm{BP}(I^{T}_{\textrm{in}}, T),T^{'})$, with twenty Residual Dense Blocks (RDBs), eight convolutional layers per RDB, and growth rate of sixty-four. The input for 2D Refiner is a concatenation of $\textrm{FP}(\textrm{BP}(I^{T}_{\textrm{in}}, T),T^{'})$ and $I^{T}_{\textrm{in}}$ to ensure both the original information and the geometric transformation are included.

\input{imgs/supplemental/suppress_alg}
\section{CT2Xray}
A more detailed visualization of CT2Xray is shown in Fig. \ref{fig:ct2xray_vis}. Given the CT volume and its bone label $\{V_{\textrm{CT}}, V_{\textrm{bone}}\}$, we can calculate for $\{V_{bone}, V_{tissue}\}$ and obtain $t^{\textrm{CT}}_{\textrm{bone}}(T), t^{\textrm{CT}}_{\textrm{tissue}}(T)$ through our proposed differential forward projection. The corresponding attenuation is then calculated and summed to produce a realistic radiograph. Compared to the original DeepDRR \cite{DBLP:conf/miccai/UnberathZLBFAN18}, CT2Xray discarded calculation for air-specific attenuation (air volume is considered as tissue), scatter estimation, and noise.
We find that air-specific attenuation calculation as followed by the measurements in \cite{hubbell1995tables} leads to a reduction in contrast on our CT dataset, and that the original CNN-based scatter estimation in DeepDRR is not robust enough on unseen data. %Lastly, instead of the full one hundred and five energy-based attenuation coefficients $\mu(m, E)$ measured in \cite{hubbell1995tables}, we selected ten energy level 
\input{imgs/supplemental/more_sim_metrics}
\section{Reversing CT2Xray for bone suppression}
Bone suppression seeks to reduce bone attenuation such that the overlapped tissue is more visible. While $t^{\textrm{ref}}_{\textrm{bone}}$ and $t^{\textrm{ref}}_{\textrm{tissue}}$ are generated from XraySyn and can be used straightforwardly to reduce bone attenuation, they do not preserve all the details in input $I^{T}_{\textrm{in}}$. Therefore, we seek to reverse CT2Xray mathematically to find a $t^{\textrm{recon}}_{\textrm{tissue}}$, such that $t^{\textrm{ref}}_{\textrm{bone}}$ and $t^{\textrm{recon}}_{\textrm{tissue}}$ reconstruct $I^{T}_{\textrm{in}}$ losslessly. As shown in Algorithm \ref{alg:reverse_CT2Xray}, we first transform $I^{T}_{\textrm{in}}$ from the range of image pixels to physical attenuation by using $I^{T}_{\textrm{atten}}$ (described in Eq. \ref{eq:ct2xray_eq}) as the reference, and obtain $I^{T}_{\textrm{inAtten}}$. We then use $t^{\textrm{ref}}_{\textrm{tissue}}$ as a reference to calculate the weight of each term in the summation over energy level $E$ that produced $I^{T}_{\textrm{atten}}$, and apply these weights on $I^{T}_{\textrm{inAtten}}$. $t^{\textrm{recon}}_{\textrm{tissue}}$ can then be calculated straightforwardly and used in the forward attenuation calculations to obtain bone-suppressed radiograph $I^{T}_{\textrm{inSupress}}$, where the attenuation coefficient of $t^{\textrm{ref}}_{\textrm{bone}}$ is reduced. A comparison of bone suppression by using $\{t^{\textrm{ref}}_{\textrm{bone}}, t^{\textrm{ref}}_{\textrm{tissue}}\}$ and $\{t^{\textrm{ref}}_{\textrm{bone}}, t^{\textrm{recon}}_{\textrm{tissue}}\}$ are shown in Fig. \ref{fig:bone_sup_supp}. 

\input{imgs/supplemental/bone_suppress}

\section{More detailed metrics on simualted data}
A more detailed view synthesis evaluation is shown in Table \ref{tab:ablation_table_supp}, where PSNR/SSIM is measured over ten different synthesized views. As we can see, view synthesis becomes less accurate with respect to the ground truth as the view angle deviates further away from the input view. This is consistent with intuition as a single view contains very limited 3D information.

\section{Additional visual results}
For additional visual results of XraySyn on radiograph view synthesis and bone suppression, please refer to the attached multi-media file.



==> XraySyn New/supplemental_material_old.tex <==
\section{Supplemental Material}


\subsection{Comparison of CT2Xray and DeepDRR}
\input{imgs/supplemental/versus}
\input{imgs/supplemental/tissue_weight}
While CT2Xray is inspired by DeepDRR, it is improved in many aspects in order to work on the task of X-ray view synthesis. Beyond the ability to propagate gradients, we show here the other aspects of improvements of CT2Xray, namely in speed and flexibility. 

The DeepDRR pipeline involves segmentation of a CT volume into three materials: bones, tissues, and air. Each material is forward projected to generate $t_{bone, tissue, air}$ and undergoes attenuation calculation. A CNN-based scatter estimation and a Poisson noise are added on top of the attenuation calculation. As shown in Fig. \ref{fig:versus}, we find that the scatter estimation CNN is not robust enough for general usage, and finetuning it requires MC simulation of X-ray images, which is infeasible to scale. Based on the results from DeepDRR, scatter estimation contributes relatively little to the overall image quality; therefore, we discard the scatter estimation. We also discard the calculation of $t_{air}$, as we find that the simulation without it bares more semblance to real X-ray images found in CheXpert, where the contrast between bone and air is significantly higher. Overall, CT2Xray is about five times faster than DeepDRR.


Since tissues consist of a wide range of materials, each with different attenuation rate, and the current CT2Xray pipeline considers all tissue as one material, there exists discrepancies between the generated X-ray image and a real X-ray image. Specifically, there is no way to modulate the contribution of $\mu_{tissue}$ in the final X-ray output when $\mu_{tissue}$ is either over-estimated or under-estimated. We therefore introduce a weight $\omega_{tissue}$ to fill this need. As shown in Fig. \ref{fig:tissue_weight}, when $\mu_{tissue}$ is clearly over-estimated for the heart region, we can lower $\omega_{tissue}$ to make it much more similar to the real X-ray input.





==> XraySyn New/tables/ablation.tex <==
\begin{table*}[t!]
\small
\centering 
\begin{tabular}{| c|c|ccc c |}
\hline
PSNR/SSIM & Loss &Volume & X-ray Orig & X-ray View 1 &  X-ray View 2 \\
% \hline
% \multirow{ 2}*{Bicubic}  & x4 &  &  &  &  &   \\
%  & x6 &  &  &  &  &  \\
\hline

X2CT-CNN\cite{DBLP:conf/cvpr/YingGMWWZ19} & $\mathcal{L}_{CT}+\mathcal{L}_{xray}$&17.57/0.5327 & 20.34/0.6787 & 19.75/0.6797 & 18.70/0.7597   \\
$\textrm{XraySyn}^{Refine}$ & $\mathcal{L}_{CT}+\mathcal{L}_{xray}$& 17.86/0.5505 & 27.05/0.9234 & 23.14/0.8175 & 18.32/0.7480\\
\hline
2D Encoder & $\mathcal{L}_{CT}+\mathcal{L}_{xray}$& 16.32/0.4360 & 18.90/0.5836 & 18.81/0.5903 & 17.98/0.6856\\
$\textrm{XraySyn}^{Refine}_{GAN}$ & $\mathcal{L}_{CT}+\mathcal{L}_{xray}+\mathcal{L}_{GAN}$& 16.91/0.4434 &23.14/0.7911 &21.34/0.7098& 18.15/0.6869\\
XraySyn & $\mathcal{L}_{CT}+\mathcal{L}_{xray}+\mathcal{L}_{code}$& 16.61/0.4522& 22.82/0.7310&21.33/0.7068 & 18.61/0.7113 \\
\hline



\hline
\end{tabular}
\vspace{-1pt}
\caption{Ablation study of XraySyn against alternative methods with quantitative evaluations. The quantitative metrics are calculated based on test data from LIDC-IDRI\cite{armato2011lung}}
\label{tab:ablation_table}
\vspace{-1pt}
\end{table*}

==> XraySyn New/tables/modified_ablation.tex <==
\begin{table*}[htb!]
\small
\centering 
\setlength\tabcolsep{1.5pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{Metrics} & 2D Refiner & 2D Encoder & X2CT-CNN & $\textrm{XraySyn}^{v1}$ & $\textrm{XraySyn}^{v2}$ & $\textrm{XraySyn}^{v3}$ & XraySyn+\\
% \hline
% \multirow{ 2}*{Bicubic}  & x4 &  &  &  &  &   \\
%  & x6 &  &  &  &  &  \\
\hline

Orig &Xray &\diagbox[innerwidth=5em, height=1.1em]{}{}& 18.90/0.584 & 20.34/0.679&22.13/0.814 &\textbf{27.05/0.923} & \underline{23.14/0.791} &22.82/0.731\\
\hline
Orig &Bone &\diagbox[innerwidth=5em, height=1.1em]{method}{view} & 17.40/0.378& 16.02/0.206&18.47/0.491 & \textbf{19.61}/0.544&19.04/\textbf{0.552} &\underline{19.24}/\underline{0.547}\\
\hline
Orig &Tissue &\diagbox[innerwidth=5em, height=1.1em]{}{} & 19.14/0.622&19.49/0.692 & \underline{21.20}/\textbf{0.766} & \textbf{21.58}/\underline{0.753}& 20.78/0.700 &20.71/0.699\\
\hline
Orig &FID &\diagbox[innerwidth=5em, height=1.1em]{}{} &\underline{0.593}& 2.388& 0.965& 0.776& 1.025 &\textbf{0.564}\\
\hline
Rand. &Xray &\underline{23.30/0.783}& 18.81/0.582& 20.01/0.675& 21.52/0.782& \textbf{24.99/0.860}& 22.62/0.766&22.13/0.717\\
\hline
Rand. &Bone &\diagbox[innerwidth=5em, height=1.1em]{}{} & 17.32/0.378& 15.90/0.204& 18.02/0.466& \textbf{19.03}/0.513& 18.96/\underline{0.530}&\underline{18.99}/\textbf{0.537}\\
\hline
Rand. &Tissue &\diagbox[innerwidth=5em, height=1.1em]{}{} & 19.22/0.625& 19.54/0.693& \underline{21.07/0.758}& \textbf{21.40/0.754}& 20.78/0.705&20.64/0.698\\
\hline
Rand. &FID & 1.779&\underline{0.585}& 2.383& 1.003& 0.873& 1.134&\textbf{0.555}\\

\hline


% X2CT-CNN\cite{DBLP:conf/cvpr/YingGMWWZ19} & $\mathcal{L}_{CT}+\mathcal{L}_{xray}$&17.57/0.5327 & 20.34/0.6787 & 19.75/0.6797 & 18.70/0.7597   \\
% $\textrm{XraySyn}^{Refine}$ & $\mathcal{L}_{CT}+\mathcal{L}_{xray}$& 17.86/0.5505 & 27.05/0.9234 & 23.14/0.8175 & 18.32/0.7480\\
% \hline
% 2D Encoder & $\mathcal{L}_{CT}+\mathcal{L}_{xray}$& 16.32/0.4360 & 18.90/0.5836 & 18.81/0.5903 & 17.98/0.6856\\
% $\textrm{XraySyn}^{Refine}_{GAN}$ & $\mathcal{L}_{CT}+\mathcal{L}_{xray}+\mathcal{L}_{GAN}$& 16.91/0.4434 &23.14/0.7911 &21.34/0.7098& 18.15/0.6869\\
% XraySyn & $\mathcal{L}_{CT}+\mathcal{L}_{xray}+\mathcal{L}_{code}$& 16.61/0.4522& 22.82/0.7310&21.33/0.7068 & 18.61/0.7113 \\


\end{tabular}
\caption{Ablation study of our proposed methods against alternative implementations. The quantitative metrics are calculated based on test data from LIDC-IDRI\cite{armato2011lung}. 2D Refiner is a purely image-to-image approach and does not involve generation of bone and tissue, therefore respective metrics are omitted.} 
\label{tab:ablation_table}

\vspace{-1em}
\end{table*}

==> XraySyn New/tables/new_ablation.tex <==
\begin{table*}[htb!]
\small
\centering 
\setlength\tabcolsep{1.5pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
% & view/method & \multicolumn{3}{|c|}{$T$} & \multicolumn{3}{|c|}{$T^{'}$}\\
\multirow{5}{*}{Simulated}  & \diagbox[innerwidth=6em, height=2em]{Method}{View} & $I^{T}_{\textrm{CT}}$ & $t^{T}_{\textrm{bone}}$ & $t^{T}_{\textrm{tissue}}$ & $I^{T^{'}}_{\textrm{CT}}$ & $t^{T^{'}}_{\textrm{bone}}$ & $t^{T^{'}}_{\textrm{tissue}}$ \\
\cline{2-8}
& 2D Refiner & \diagbox[innerwidth=5em, height=1.1em]{}{} & \diagbox[innerwidth=5em, height=1.1em]{}{} & \diagbox[innerwidth=5em, height=1.1em]{}{} & 21.09/0.801 & \diagbox[innerwidth=5em, height=1.1em]{}{} & \diagbox[innerwidth=5em, height=1.1em]{}{}\\
\cline{2-8}
& X2CT & 20.44/0.755 & 15.99/0.451 & 19.57/0.711 & 20.20/0.750 & 16.12/0.450 & 19.38/0.703\\
\cline{2-8}
& 3DPN-DRR & 21.05/0.925 & \diagbox[innerwidth=5em, height=1.1em]{}{} & \diagbox[innerwidth=5em, height=1.1em]{}{} & 19.79/0.867 & \diagbox[innerwidth=5em, height=1.1em]{}{} & \diagbox[innerwidth=5em, height=1.1em]{}{}\\
\cline{2-8}
& 3DPN & 29.49/0.961 & 22.30/0.814 & 24.40/0.866 & 27.22/0.929 & 21.63/0.780 & 24.27/0.860\\
\hline
\multirow{4}{*}{Real} & \diagbox[innerwidth=6em, height=2em]{Method}{View} & \multicolumn{3}{c|}{$I^{T}_{\textrm{final}}$} & \multicolumn{3}{c|}{$I^{T^{'}}_{\textrm{final}}$(FID only)}\\
% \cline{2-8}
% & 3DPN-DRR &  \multicolumn{3}{c|}{}  & \multicolumn{3}{c|}{} \\
\cline{2-8} 
& 3DPN &  \multicolumn{3}{c|}{22.75/0.819}  & \multicolumn{3}{c|}{1.09} \\
\cline{2-8}
& $\textrm{XraySyn}^{\textrm{no}\mathcal{M}}$ &  \multicolumn{3}{c|}{28.42/0.857}  & \multicolumn{3}{c|}{0.375} \\
\cline{2-8}
& XraySyn & \multicolumn{3}{c|}{30.33/0.865}  & \multicolumn{3}{c|}{0.319} \\

\hline

\end{tabular}
\caption{Ablation study of our proposed methods against alternative implementations. Note that 3DPN-DRR and 2D Refiner do not use CT2Xray, therefore are without metrics for $t_{\textrm{bone}}$, $t_{\textrm{tissue}}$. $I^{T}_{\textrm{CT}}$ for 2D Refiner is trivially generated as $I^{T}_{\textrm{in}}$. PSNR/SSIM metrics are provided when groundtruth is available, otherwise FID score is reported. The best performing metrics are \textbf{bold}, the second best metrics are \underline{underlined}.} 
\label{tab:ablation_table}

\vspace{-1em}
\end{table*}

==> XraySyn New/tables/newer_ablation.tex <==
\begin{table*}[htb!]
\small
\centering 
\setlength\tabcolsep{1.5pt}
\begin{tabular}{|l|c|c|c|c|c|c|c|l|c|c|}
\hline
% & view/method & \multicolumn{3}{|c|}{$T$} & \multicolumn{3}{|c|}{$T^{'}$}\\
\multicolumn{7}{|c|}{Simulated} && \multicolumn{3}{c|}{Real}\\
\hline
\diagbox[innerwidth=6em, height=2em]{Method}{View} & $I^{T}_{\textrm{CT}}$ & $t^{T}_{\textrm{bone}}$ & $t^{T}_{\textrm{tissue}}$ & $I^{T^{'}}_{\textrm{CT}}$ & $t^{T^{'}}_{\textrm{bone}}$ & $t^{T^{'}}_{\textrm{tissue}}$ && \diagbox[innerwidth=6em, height=2em]{Method}{View} & $I^{T}_{\textrm{final}}$ & $I^{T^{'}}_{\textrm{final}}$ (FID) \\
% \cline{2-7}
\hline
2D Refiner & \diagbox[innerwidth=5em, height=1.1em]{}{} & \diagbox[innerwidth=5em, height=1.1em]{}{} & \diagbox[innerwidth=5em, height=1.1em]{}{} & 21.09/0.801 & \diagbox[innerwidth=5em, height=1.1em]{}{} & \diagbox[innerwidth=5em, height=1.1em]{}{} & &3DPN & 22.75/0.819  & 1.090\\
% \cline{2-7}
\hline
X2CT & 20.44/0.755 & 15.99/0.451 & 19.57/0.711 & 20.20/0.750 & 16.12/0.450 & 19.38/0.703 &&$\textrm{XraySyn}^{\textrm{no}\mathcal{M}}$ &  28.42/0.857  & 0.375\\
% \cline{2-7}
\hline
3DPN-DRR & 21.05/0.925 & \diagbox[innerwidth=5em, height=1.1em]{}{} & \diagbox[innerwidth=5em, height=1.1em]{}{} & 19.79/0.867 & \diagbox[innerwidth=5em, height=1.1em]{}{} & \diagbox[innerwidth=5em, height=1.1em]{}{}& &XraySyn & \textbf{30.33/0.865}  & \textbf{0.319} \\
% \cline{2-7}
\hline
3DPN & \textbf{29.49/0.961} & \textbf{22.30/0.814} & \textbf{24.40/0.866} & \textbf{27.22/0.929} & \textbf{21.63/0.780} & \textbf{24.27/0.860} && & &\\
\hline
% \cline{2-7}
% & 3DPN-DRR &  \multicolumn{3}{c|}{}  & \multicolumn{3}{c|}{} \\
% \cline{2-7} 
% \cline{2-7}
% \cline{2-7}

\end{tabular}
\caption{Ablation study of our proposed methods against alternative implementations. Note that 3DPN-DRR and 2D Refiner do not use CT2Xray, therefore are without metrics for $t_{\textrm{bone}}$, $t_{\textrm{tissue}}$. $I^{T}_{\textrm{CT}}$ for 2D Refiner is trivially generated as $I^{T}_{\textrm{in}}$. PSNR/SSIM metrics are provided when groundtruth is available, otherwise FID score is reported. The best performing metrics are \textbf{bold}.} 
\label{tab:ablation_table}

\vspace{-1em}
\end{table*}

==> abstract.tex <==
\begin{abstract}

X-ray view synthesis has seldom been studied compared to its natural image counterpart due to various prohibitive challenges. Firstly, multi-view X-ray images are rare due to the invasive acquisition process, and X-ray simulations are either unrealistic or computationally expensive. Secondly, the material-penetrating nature of X-ray means that synthesizing from different views requires 3D knowledge of both the surface and internal of the subject. Lastly, as materials attenuate differently, dense but small details such as bones have a large impact on synthesized X-ray images but are hard to generate realistically. In this work, we conceive a differentiable projectior algorithm, named CT2Xray, to efficiently generate realistic X-ray simulations from CT volumes, thus resolving the first challenge. We also propose an end-to-end X-ray view synthesis algorithm called $\textit{XraySyn}$, which is able to synthesize X-ray views with high realism. We further show that XraySyn performs robustly on real X-ray images without extra steps for domain adaptation. To the authors' best knowledge, this is the first work on realistic X-ray image view synthesis. Code will be made available on GitHub.



\end{abstract}

==> experiment_backup.tex <==
\section{Experiments}

\input{tables/modified_ablation}
\subsection{Dataset}
As there exists no public dataset that contains either aligned, multi-view X-ray data, or geometrically paired X-ray and CT data, we use CT volumes and our proposed CT2Xray operator to simulate these relationships. Specifically, we use the LIDC-IDRI dataset \cite{armato2011lung}, which contains
1,018 chest CT volumes, for simulation. To preprocess the LIDC-IDRI data, we resample the CT volumes to a uniform voxel resolution of $2\times2\times2\textrm{mm}^3$ and crop a central region of $256\times256\times256\textrm{mm}^3$ from each CT scan. Furthermore, we discards all volumes that have a between-slices resolution higher than 2.5mm. This leads to 780 CT volumes, where we randomly select 700 for training, 10 for evaluation, and 70 for testing. To show the robustness of our method on real images, we select a number of suitable X-ray images from CheXpert \cite{DBLP:conf/aaai/IrvinRKYCCMHBSS19} for testing.


%  As shown in Figure. 2, such simulation is done at online training, where the only required input

%Proper preprocessing steps, such as rotating and cropping, are taken to ensure the real X-ray images are geometrically similar with simulated X-ray images from the training dataset.

%explain the experiment setup as simulations, i.e. the entire pipeline

\subsection{Implementation Details}
As shown in Figure. 2, at each training iteration, a CT volume $V_{CT}$ is used to simulate the groundtruth X-ray images from view rotations $T, T^{'}$. All simulated X-ray images generated from the CT2Xray operator are normalized to range between 0 and 1. We find thresholding to be the most robust method to separate bone and tissues in any given CT volume, as well as computationally inexpensive. For simulation during training, we randomly select the hyperparameter $\omega_{tissue}$ to be between 0.8 to 1.2 and clip the dynamic range of the generated $I_{Xray}$ from 70 to 100$\%$ to simulate for different real X-ray images. We further select $T$ and $T^{'}$ randomly from -18$\degree$ to 18$\degree$ in azimuth and elevation angles. For simulation during testing, $\omega_{tissue}$ is set to be 0.8, and image dynamic range is clipped at 90$\%$. We set $\lambda_{in} = 1.0$ and $\lambda_{new} = 0.25$ for $\mathcal{L}^{G, F}_{xray}$, and $\lambda_{CT} = \lambda_{xray} = 1.0$. Due to the discretization of a voxel-based representation in digital system, the ray tracing process used in forward and backprojection can only approximates points in space when those points are not on integer coordinates. We use trilinear interpolation for such approximation. For more details about implementation, please refer to the supplemental material.


\subsection{Evaluation Metrics}
There are several different factors involved with evaluating the effectiveness of X-ray view synthesis. Firstly, as the input X-ray image is the only reliable data about the subject, one goal is to ensure that such information is preserved during the proposed 2D-to-3D inversion. To this end, we use Peak Signal-to-Noise Ratio (PSNR) and Structured Similarity Index (SSIM) to measure the overall recovery of the input X-ray image. To address the aspect of recovering realistic anatomical details, we measure the PSNR/SSIM value of $t(tissue)$ and $t(bone)$ for the input and output X-ray images of the same view. Lastly, Fréchet Inception Distance (FID) is used as a metric to measure realism of the generated X-ray images. We make two adaptions to FID for X-rays: 1. repeating the grayscale values across the RGB channels as the pre-trained InceptionV3 model works on RGB images; 2. calculating the FID score by using the middle layers of InceptionV3, specifically the 768-channel layer before InceptionV3's last auxiliary classifier, for lower level features. The same evaluation metrics are calculated for synthesized views over a set of 10 angles, which are uniformly selected -18$\%$ to 18$\%$ azimuthally from the input view angle. 


\input{imgs/ablation}
\subsection{Ablation Study}
We evaluate the effectiveness of XraySyn 1. against alternative 2D or 3D implementations, and 2. over different training loss setups. Specifically, comparisons are made between the following setups: 

\begin{enumerate}[label=\Alph*),itemsep=1 pt]
    \item 2D Refiner: A baseline image-to-image method by synthesizing new views from input $FP(BP(I^{T}_{in}, T),T^{'})$ through a 2D DenseNet structure. The training is constrained a L1 loss between the generated X-ray and its groundtruth. 
    \item 2D Encoder: A 2D DenseNet structure that directly projects $I^{T}_{in}$ onto the latent space of the chest CT PGGAN.The training losses are consistent with Eq. \ref{eqn:loss+} with $\lambda_{CT}=1.0$, $\lambda_{Xray}=0.25$, and no $\mathcal{L}_{code}$. 
    \item X2CT-CNN: Proposed by Ying et al. to transform DRRs into CT volumes. We made the following adaptations: 1. instead of DRRs, the inputs are X-rays generated by CT2Xray, and 2. the training losses are consistent with Eq. \ref{eqn:loss}, where $\lambda_{CT}=1.0$, $\lambda_{Xray}=0.25$, $\lambda_{GAN}=0.0$;
    \item $\textrm{XraySyn}^{v1}$: XraySyn with $\lambda_{CT}=1.0$, $\lambda_{Xray}=0.0$, $\lambda_{GAN}=0.0$;
    \item $\textrm{XraySyn}^{v2}$: XraySyn with $\lambda_{CT}=1.0$, $\lambda_{Xray}=0.25$, $\lambda_{GAN}=0.0$;
    \item $\textrm{XraySyn}^{v3}$: XraySyn with $\lambda_{CT}=1.0$, $\lambda_{Xray}=0.25$, $\lambda_{GAN}=0.01$;
    \item XraySyn+: XraySyn+ with $\lambda_{CT}=1.0$, $\lambda_{Xray}=0.25$, $\lambda_{code}=0.1$.
\end{enumerate}


Table \ref{tab:ablation_table} summarizes the performance of different implementations over various view angles, visualization of the results are provided in Fig. \ref{tab:ablation_img}. As shown, image-to-image approach like 2D Refiner generates synthesized view as mostly a blurry version of the input view. The lack of an intermediary 3D structure forces the network to account for the variations by overly smoothing the output to achieve a lowest pixel-wise loss. X2CT-CNN copies the features in 2D along the third axis to achieve the initial upsampling from 2D to 3D, which is geometrically incorrect for arbitrary view angle. While we find that CNN's strong curve-fitting ability still leads X2CT-CNN to produce reasonable 3D estimation, it cannot learn the complex geometric transformation that maps the input image to the correct view; therefore, the synthesized views are entirely reliant on the 3D structure and lack significant details, as shown in Fig. \ref{tab:ablation_img}. 

We show that by using the geometrically consistent backprojection and CT2Xray operators, XraySyn and XraySyn+ excel in preserving the input X-ray view in their generated CT volume. Specifically, we examine XraySyn with different loss setups to observe the utility of each loss component. $\textrm{XraySyn}^{v1}$ is trained with only $\mathcal{L}^{G}_{CT}$ to best approximate the original CT volume. Due to the ill-posed nature of 2D-to-3D conversion, however, the generated CT volume can still be very different from the groundtruth, as shown in Fig. \ref{tab:ablation_img}. By adding the $\mathcal{L}^{G}_{xray}$ term in training $\textrm{XraySyn}^{v2}$, we explicitly enforces the preservation of the input X-ray view, which leads to significantly better synthesized images metrically and visually, specifically on the recovery of bone structures. We further observe that both results from $\textrm{XraySyn}^{v1}$ and $\textrm{XraySyn}^{v2}$ are lacking in a realistic bone structure, which is also evident in CT. $\textrm{XraySyn}^{v3}$ adds a LSGAN component to the loss formulation to promote more realistic recovery of bone structures. It can be observed that $\textrm{XraySyn}^{v3}$ produces a better bone-tissue contrast in CT, but is unable to reach satisfactory definition in details. Overall, XraySyn performs well at generating the 3D volume that preserves the original X-ray input in terms of PSNR, with some deficiency in generating bone details.

\input{imgs/real_results}
XraySyn+ is introduced to address this issue. By leveraging the underlying manifold found through 3D PGGAN, XraySyn+ is able to generate realistic CT volume with a clear bone structure. For comparison, an alternative 2D Encoder is implemented to directly projects the input X-ray image onto the chest CT manifold. We find that the lack of auxiliary constraint like $\mathcal{L}_{code}$, along with the limited input information in 2D, leads 2D Encoder to find sub-optimal solutions. XraySyn+ performs much better than 2D Encoder in terms of PSNR/SSIM, while providing much more realistic X-ray images both visually and according to the FID scores. On the other hand, due to various challenges in GAN inversion and the limited data used to train a PGGAN, XraySyn+ is constrained in its ability to produce images that are as pixel-wise consistent as $\textrm{XraySyn}^{v2}$. However, we find the bone and tissue-wise metrics for XraySyn+ and $\textrm{XraySyn}^{v2}$ are much more similar, suggesting that part of the difference in X-ray PSNR/SSIM metrics is due to the the segmentation component in CT2Xray. In general, we find that the imperfections of segmentation methods lead to favorable X-ray PSNR/SSIM measurements for $\textrm{XraySyn}^{v2}$, as the CT volume produced by $\textrm{XraySyn}^{v2}$ is smoother and less noisy when segmented. In comparison PGGAN produced CT volumes are much more detailed and more difficult to segment properly. 

Lastly, we note that comparisons for synthesized non-input views are difficult. While measurements with respect to views generated from the groundtruth volume can serve as a guidance, they should be considered with the understanding that no method can recover the exact volume since 2D-to-3D inversion is a one-to-many mapping. This demonstrates the difficulties in X-ray view synthesis. In general, we find that XraySyn produces more voxel-wise accurate CT volume and thus pixel-wise accurate X-ray images; however, as the view angle shifts further away from the input view, more bone structure may be missing. In contrast, XraySyn+ produces less voxel-wise accurate CT volume, but realistic X-ray images regardless of the view angle.

% While it is expected that metrics like PSNR/SSIM for XraySyn+'s synthesized views are worse compared to $\textrm{XraySyn}^{v2}$, as is often observed in GAN-based super-resolution literature, we find that the bone and tissue-wise metrics for XraySyn+ and $\textrm{XraySyn}^{v2}$ are much more similar. As the generation of X-ray images is based on segmentation of bone and tissues, the pixel-wise consistency between X-ray images is heavily influenced by whether the segmentation outcomes are consistent or not. In general, we find that the imperfections of segmentation methods lead to favorably X-ray PSNR/SSIM measurements for $\textrm{XraySyn}^{v2}$ compared to XraySyn+, as the CT volume produced by $\textrm{XraySyn}^{v2}$ is smoother and less noisy when segmented. Lastly, FID is significantly better for X-ray images generated by XraySyn+ and 2D Encoder, showing that these images are highly realistic. 




% Since X2CT-CNN upsamples 2D image to 3D by repeating the pixel values over the third dimension, the generated volume cannot preserve the original X-ray image and are fully relied on the generated volume. $\textrm{XraySyn}^{Ref}$ generates CT volumes based on $V_{BP}$, which places the X-ray image in 3D according to cone-beam geometry, and has significantly improved performance generating X-ray images over the same view. Despite such a advantage, both methods are unable to generate global details like the bone structure, as is evident in the lateral view. $\textrm{XraySyn}^{Ref}_{GAN}$ adds a GAN Loss to introduce more details in the generated volume; as we can see in Fig. \ref{tab:ablation_img}, constrained by $\mathcal{L}_{CT}$, $\mathcal{L}_{xray}$, and $\mathcal{L}_{GAN}$, $\textrm{XraySyn}^{Ref}_{GAN}$ generates volumes that has mediocre performance in preserving the original X-ray image and generating 3D details. 2D Encoder uses a trained PGGAN to generate 3D Volume, therefore the resulting volume is much more realistic; however, due to the lack of constraint over the latent code and the under-constrained 2D-to-3D condition, 2D Encoder predicts latent codes that are very far away from the normal distribution used to train PGGAN, i.e. gets easily trapped in local minimums. As a result, not only does it underperform during training, 2D Encoder benefits very little from individual fine-tuning. In comparison, XraySyn incorporates the benefits of both $\textrm{XraySyn}^{Ref}$ and 2D Encoder, where it can generate reliable same-view X-ray image, and a highly detailed CT volume.

\subsection{XraySyn+ on Real X-ray Images}
In this section, we exam XraySyn+'s performance on real X-ray images. There are many hyperparameters related to view synthesis, including the unknown input view angle $T$, the distance between X-ray source to detector, the dynamic range of the X-ray images, etc. To accurately estimate these hyperparameters is out of the scope of this paper. In this paper, we roughly estimate these hyperparameters by 1. cropping and rotating the original X-ray image into regions that are similar to the training dataset, and 2. search through a small interval of view transform $T$ on the output CT to find a $T$ that achieves the highest PSNR value between the generated and observed X-ray image. 

Fig. \ref{img:real_results} shows the visual results of XraySyn+ on real X-ray images. As we can see, XraySyn+ does a fairly good job at preserving the overall anatomy, indicating that simulated X-ray images generated through CT2Xray are effective at capturing X-ray characteristics. The new views can provide users with knowledge of how organs, e.g. the heart and lung, are shaped in 3D. We observe that there are some discrepancies between real and generated X-ray images, especially at the lower, abdominal section where shadows in the real X-ray images are not represented. This may be due to 1. the abdominal section is not well represented in the limited chest CT dataset, and 2. the material in the abdominal section is not well modelled in CT2Xray. As the training dataset expands to cover more human anatomy and better separation at different materials, we posit that the results will be much improved. 



==> imgs/ablation.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}[b]{|ccccccccc|}
        \hline
        View & 2D Refiner & 2D Encoder & X2CT-CNN &  $\textrm{XraySyn}^{v1}$ &$\textrm{XraySyn}^{v2}$ & $\textrm{XraySyn}^{v3}$ &  XraySyn+ & G.T. \\
        Input View & 
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/2d_refiner/2_5_pred.png}
            \caption{22.6/\textbf{0.93}/0.79}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/2d_encoder/2_pred_in.png}
            \caption{18.2/0.61/\textbf{0.48}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/x2ct-cnn/2_pred_in.png}
            \caption{21.9/0.74/2.46}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/3d_only/2_pred_in.png}
            \caption{\underline{24.9}/0.85/1.25}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/unet-l1/2_pred_in.png}
            \caption{\textbf{27.1}/\underline{0.91}/0.92}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/unet-gan/2_pred_in.png}
            \caption{23.9/0.80/1.26}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/xraysyn-refine/2_pred_in.png}
            \caption{24.0/0.78/\underline{0.55}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/2_orig_in.png}
            \caption{\phantom{}}
        \end{subfigure} \\  
        9$\degree$ View & 
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/2d_refiner/2_8_pred.png}
            \caption{22.9/\underline{0.82}/1.87}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/2d_encoder/2_8_pred.png}
            \caption{17.7/0.58/\underline{0.56}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/x2ct/2_8_pred.png}
            \caption{20.7/0.71/2.42}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/xraysyn_v1/2_2_pred.png}
            \caption{\underline{23.2}/0.81/1.11}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/xraysyn_v2/2_8_pred.png}
            \caption{\textbf{24.8/0.85}/1.03}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/xraysyn_v3/2_2_pred.png}
            \caption{22.9/0.78/1.29}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/xraysyn+/2_8_pred.png}
            \caption{22.5/0.76/\textbf{0.43}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/orig/2_8_orig.png}
            \caption{\phantom{}}
        \end{subfigure} \\   
        18$\degree$ View & 
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/new_imgs/2d_refiner/2_10_pred.png}
            \caption{21.2/0.75/2.12}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/2d_encoder/2_pred_gt1.png}
            \caption{16.3/0.56/\underline{0.41}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/x2ct-cnn/2_pred_gt1.png}
            \caption{19.5/0.69/2.51}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/3d_only/2_pred_gt1.png}
            \caption{\underline{22.5}/0.79/0.96}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/unet-l1/2_pred_gt1.png}
            \caption{\textbf{22.8/0.81}/0.88}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/unet-gan/2_pred_gt1.png}
            \caption{20.8/\underline{0.81}/0.88}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/xraysyn-refine/2_pred_gt1.png}
            \caption{20.0/0.73/\textbf{0.33}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/2_orig_gt1.png}
            \caption{\phantom{}}
        \end{subfigure} \\           
        Lateral CT & 
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/blank.png}
            % \caption{14.02/0.3496}
        \end{subfigure} &
        % \diagbox[innerwidth=5em, height=5em]{}{} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/2d_encoder/2_pred_vol.png}
            % \caption{14.02/0.3496}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/x2ct-cnn/2_pred_vol.png}
            % \caption{14.25/0.4601}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/3d_only/2_pred_vol.png}
            % \caption{14.02/0.3496}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/unet-l1/2_pred_vol.png}
            % \caption{15.22/0.4859}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/unet-gan/2_pred_vol.png}
            % \caption{14.19/0.3392}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/xraysyn-refine/2_pred_vol.png}
            % \caption{14.50/0.3902}
        \end{subfigure} &
        \begin{subfigure}[b]{0.11\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/2_orig_vol.png}
            % \caption{PSNR/SSIM}
        \end{subfigure} \\     
        \hline
    \end{tabular}
    \caption{Visual comparisons of X-ray images generated by different methods from different views. View angle change is measured azimuthally. For each non-groundtruth image, PSNR (higher is better), SSIM (higher is better), and FID (lower is better) are provided as metrics. We also provide a lateral image of the generated CT volume for visualization. The best performer is \textbf{bold}, the second best is \underline{underlined}.}
    \label{tab:ablation_img}
\end{figure*}

==> imgs/ablation_real.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}[b]{|cccccccc|}
        \hline
        View & -9$\degree$ & -6$\degree$ & -3$\degree$ & 0$\degree$ (Input) & 3$\degree$ & 6$\degree$ & 9$\degree$  \\
        3DPN & 
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/xray_pred_0.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/xray_pred_3.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/xray_pred_6.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/xray_pred_10.png}
            \caption{20.80}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/xray_pred_14.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/xray_pred_17.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/3dpn/xray_pred_20.png}
            \caption{}
        \end{subfigure} \\   
        XraySyn w/o $\mathcal{M}$ & 
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/xray_orig_0.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/xray_orig_3.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/xray_orig_6.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/xray_orig_10.png}
            \caption{22.06}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/xray_orig_0.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/xray_orig_0.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn_orig/xray_orig_20.png}
            \caption{}
        \end{subfigure} \\   
        XraySyn & 
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/xray_meta_0.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/xray_meta_0.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/xray_meta_0.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/xray_meta_10.png}
            \caption{29.92}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/xray_meta_14.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/xray_meta_17.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xraysyn/xray_meta_20.png}
            \caption{}
        \end{subfigure} \\ 
        Groundtruth & 
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/blank.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/blank.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/blank.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation_real_case6/xray_orig.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/blank.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/blank.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/ablation/blank.png}
        \end{subfigure} \\
        \hline
    \end{tabular}
    \caption{Visual comparisons of X-ray images generated by different methods from different views. View angle change is measured azimuthally. For each non-groundtruth image, PSNR (higher is better), SSIM (higher is better), and FID (lower is better) are provided as metrics. We also provide a lateral image of the generated CT volume for visualization. The best performer is \textbf{bold}, the second best is \underline{underlined}.}
    \label{tab:ablation_img_real}
\end{figure*}

==> imgs/intro_img.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\vspace{-5em}
\begin{center}
    \centering
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/xray_meta_0.png}
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/xray_meta_5.png}
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/xray_orig.png}
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/xray_meta_15.png}
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/xray_meta_20.png}\\
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/bone_refine_0.png}
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/bone_refine_5.png}
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/bone_refine_10.png}
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/bone_refine_15.png}
    \includegraphics[width=.195\textwidth,height=.195\textwidth]{imgs/intro_img2/bone_refine_20.png}
    % \includegraphics[width=.15\textwidth,height=.15\textwidth]{imgs/intro_img/xray_meta_195.png}
    \captionof{figure}{XraySyn can synthesize novel view radiographs from \emph{real} radiograph inputs, as shown in the first row, where the middle radiograph is the input. In addition, XraySyn also obtains the bone structure within the synthesized views, as shown in the second row. Both synthesized views and their bone structure are generated without direct supervision. For animated results, please refer to the supplemental material.}
\end{center}%
}]

==> imgs/real_results.tex <==
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}[b]{|cccc|cccc|}
        \hline
        Orig Image & Input View & 18$\degree$ View & 36$\degree$ View & Orig Image & Input View & 18$\degree$ View & 36$\degree$ View\\
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/10_orig.png}
            \caption{Case 1}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/10_input.png}
            \caption{22.08/0.7326}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/10_view1.png}
            \caption{--/--}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/10_view2.png}
            \caption{--/--}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/5_orig.png}
            \caption{Case 2}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/5_input.png}
            \caption{22.31/0.6975}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/5_view1.png}
            \caption{--/--}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/5_view2.png}
            \caption{--/--}
        \end{subfigure} \\
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/7_orig.png}
            \caption{Case 3}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/7_input.png}
            \caption{21.55/0.6943}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/7_view1.png}
            \caption{--/--}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/7_view2.png}
            \caption{--/--}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/23_orig.png}
            \caption{Case 4}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/23_input.png}
            \caption{21.07/0.7099}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/23_view1.png}
            \caption{--/--}
        \end{subfigure} &
        \begin{subfigure}[b]{0.12\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/real_imgs/23_view2.png}
            \caption{--/--}
        \end{subfigure}   \\
        
        \hline
    \end{tabular}
    \caption{View synthesis on real X-ray images. Three views, including the estimated input view and two new views 18$\degree$ and 36$\degree$ azimuthally from the input views are also shown. Some uneven intensity is introduced in alternative views due to the ellipsoid shape of human anatomy. PSNR/SSIM values are provided over the input view.}
    \label{img:real_results}
    \vspace{-1em}
\end{figure*}

==> introduction.tex <==
\section{Introduction}
In the natural image domain, single image view synthesis aims to generate an image of a scene from different viewpoints based on what is observed. Such a task can be formulated as an ill-posed, 2D-to-3D-to-2D problem, and is widely studied in the computer vision and graphics community with the recent advances in Convolutional Neural Networks (CNNs). In general, current single image view synthesis methods can be categorized into two classes, the image-to-image approach and the 3D shape generation approach. Image-to-image methods transform the observed image into an image from a desired view point, either directly or through geometric manipulations. 3D shape generation methods aim to generate a 3D model of the observed object, which can then be rendered from any other viewpoint. Due to the challenging and under-constrained nature of the problem setting, current methods are limited in either the small variability in viewing angle, the detail level of the 3D object, or both.  
%View synthesis has use cases in scene understanding, image editing, and virtual reality. 

Clinical radiographs or X-ray images are formed by applying high energy radiation through the human body, and measuring the attenuated radiation on the other side. The rate of attenuation for every ray yields a pixel value, and in aggregate forms an image that reveals subject's internal anatomy. While X-ray imaging is quick and economic, high energy radiation can cause adverse health effects. As a result, typically only a single X-ray image is taken per session regardless the fact that some radiology readings/analysis may only possible under different views. Therefore, it leads to the need for X-ray view synthesis from a single image, both for clinical use cases and for data-hungry, automated tasks such as X-ray landmark detection, registration, disease identification, etc.


% while 2D-to-3D approaches  
% 3D understanding by generating the desired 3D representation, i.e. 3D shape generation/completion, 2D-3D inversion. Typically, this type of method can only generate surface shape of simple 3D objects.
% and 2. geometrically rotate 2D image based on view angle difference, and compensate the missing information through 2D inpainting [https://arxiv.org/pdf/2004.04727v2.pdf].

Unfortunately, the differences between the imaging physics of X-ray images and natural images make the view synthesis of X-ray images even more challenging than its natural image counterpart. As X-ray can penetrate materials well, the 2D-to-3D inversion step requires the generation of the subject's surface and internal information, which increases the difficulty of the task and renders efficient 3D surface representations such as mesh, point cloud, signed distance function (SDF), etc. inapplicable. Furthermore, due to material-dependent attenuation, small but dense structures like bones are disproportionally represented in X-ray images, which necessitate the inferred 3D information to express fine details. Lastly, as the 2D images are related to a much larger 3D space, small view angle changes lead to significant variation in pixel values, which limits the effectiveness of Image-to-Image methods. These challenges, along with limited data of different views, lead to few works into X-ray view synthesis despite its apparent value. 

Fortunately, there exists a suitable, voxel-based 3D representation that has intrinsic connections to X-ray images. Computational Tomograph (CT), more specifically Cone Beam CT (CBCT), is acquired by measuring 2D X-ray attenuation over many angles and performing 3D reconstruction \cite{Feldkamp:84} to generate a volumetric image. While the 3D reconstruction step is a lossy process, therefore making the relationship between CBCT and X-ray image imprecise, if proper geometric correspondence can be established, the transformation between two domains can be approximated in a data-driven way. We show that our X-ray-to-CT-to-X-ray approach with supervised knowledge in both domains, called XraySyn, can lead to realistic results. To enable application on real data, we take special care to ensure the X-ray simulation is realistic and the resulting models are applicable to real data. In summary, our contribution can be described in four parts:

\begin{enumerate}
    \item We propose a differentiable forward projector called CT2Xray, an operator capable of converting 3D CT to realistically simulated 2D X-rays in real time, therefore providing an efficient solution to establish geometric correspondence between the CT and X-ray domains.
    \item We propose a Unet-based method called XraySyn, which is capable of generating a CT volume based on a single X-ray image. The generated CT is constrained to express the input X-ray image, and can be used to synthesize alternative views.
    \item We propose XraySyn+, which leverages PGGAN to enable realistic generation of detailed anatomical features like the bone structure;
    \item We test our approach on both simulated X-ray images from LIDC \cite{armato2011lung} and real X-ray images from CheXpert \cite{DBLP:conf/aaai/IrvinRKYCCMHBSS19}, and show that it performs robustly on both datasets.
\end{enumerate}









% While the 3D reconstruction step is a lossy process, thereby making the connection between CBCT and X-ray image imprecise, many works have relied on CBCT-generated X-ray simulations, called Digitally Reconstructed Radiographs (DRRs). 




%DRRs are generated by ray tracing through the CBCT volume and summing over the voxel values along the ray, where the voxel values are used as proxies to real attenuation values. 



%While DRRs are computationally inexpensive to generate, they are poor simulations of actual 


% Alternatively, a popular method to simulate X-ray images in silico is based on Computational Tomography, or CT. CT, particularly with cone-beam geometry(CBCT), measures 2D X-ray attenuation of the human body over many angles, and subsequently performs 3D reconstruction\cite{Feldkamp:84} to generate an image of the subject in 3D. As the 3D reconstruction is a lossy process, the connection between CT and X-ray image is imprecise. Regardless, Digitally Reconstructed Radiographs (DRRs) can be generated from CT by projecting the CT voxel values onto a 2D plane in a given direction, and are used as inaccurate but computationally inexpensive X-ray simulations. 





==> method_backup.tex <==
\section{Method}
At the core of our proposed methods is a differentiable forward projector called the \textit{CT2Xray} operator. To our best knowledge, the CT2Xray operator is \textit{the first algorithm} that can generate realistic X-ray images from a CT volume in a \textit{differentiable} and \textit{fast} fashion along arbitrary viewpoint. Combined with the backprojection operator, which projects X-ray images onto 3D space, these two operators help complete the cycle of transformation between the X-ray and CT domain. We then introduce XraySyn, which leverages the cycle transformation to train an end-to-end X-ray view synthesis model, and XraySyn+, which addresses the challenges in generating realistic anatomic structures.
\begin{figure*}[htb]
\centering
\includegraphics[width=\textwidth]{XraySyn_net.png}
\caption{The differentiable CT2Xray projection algorithm. CT2Xray is differentiable, fast enough to be used for online training, and generates highly realistic X-ray simulations.}
\label{fig:projector}
\end{figure*}
% A big challenge in tackling the X-ray view synthesis problem is that real, properly aligned multi-view X-ray images are rare due to the ALARA principle at acquisition; datasets such as CheXpert\cite{DBLP:conf/aaai/IrvinRKYCCMHBSS19} and others provide at most two X-ray views, which are orthogonal to each other and poorly aligned. In this paper, we perform experiments on realistically simulated X-ray images from CT volumes, and prove the effectiveness of our method by applying it on real X-ray images at test time. To this end, we first introduce a realistic and differentiable projection algorithm called CT2Xray in section \ref{sec:ct2xray}, and the view synthesis XraySyn algorithm in section \ref{sec:xraysyn}.
\subsection{CT2Xray operator}
The CT2Xray operator is explained in two parts: (i) the core differentiable forward projection algorithm; (ii) the X-ray simulation algorithm, which along with the first part forms the CT2Xray operator that directly transforms a CT volume into realistic X-ray simulations.


\textbf{Differentiable Forward Projector}.
Let $V_{CT}$ denote a CT image, the forward projector generates a 2D projection of $V_{CT}$ by:
\begin{align} \label{eq:drr}
\begin{aligned}
    I(x) = FP(V_{CT}) = \int 
    V_{CT}(T^{-1} p) d\bm{l}(x) \\
     ~\approx \sum_{p \in \bm{l}(x)} V_{CT}(T^{-1} p) \Delta p
\end{aligned}
\end{align}
where $T$ is a homogeneous matrix that controls the rotation and translation of the view point and $\bm{l}(x)$ is a line segment connecting the simulated x-ray source and detector at $x$. For backpropagation, the gradients of $I$ with respect to $V_{CT}$ can be written as
\begin{equation}\label{eq:grad}
 \dfrac{\partial I(x)}{\partial V_{CT}(y)} =
 \begin{cases}
  \Delta p, &\text{if} ~~ Ty \in \bm{l}(x),\\
     0, &\text{otherwise. }
 \end{cases}
\end{equation}
Calculations for (\ref{eq:drr}) and (\ref{eq:grad}) can be done through massive parallelism with GPUs, where every line integral over the volume is standalone%a standalone process
; as such this implementation can be used in online training.

\textbf{CT2Xray}.\label{sec:ct2xray}
Forward projecting on CT volumes generates DRRs, which are poor simulations of X-ray images due to the inaccurate assumptions. Inspired by DeepDRR \cite{DBLP:conf/miccai/UnberathZLBFAN18}, we incorporate the differentiable forward projector into a more realistic X-ray simulation pipeline, called CT2Xray. Unberath et al. proposes that a realistic X-ray attenuation $I_{atten}$ can be modeled as
\begin{align}
    I_{atten} = \sum_{E}I_{0}e^{-\sum_{m}\mu(m, E)t(m)} + SE + noise,
\end{align}
where $\mu(m, E)$ is the linear attenuation coefficient of material $m$ at energy state $E$, $t(m)$ is the material thickness, $SE$ is the estimation term that models X-ray scattering, and $I_{0}$ is the source X-ray intensity. For simplicity, $I_{0}$ is considered at the unit intensity. By first separating $V_{CT}$ into different materials $V_{m}$, our differentiable forward projector can be used to calculate $t(m)$, where $t(m) = FP(V_{m})$. %, thus making the calculation of $I_{atten}$ differentiable. 
 CT2Xray discards the calculations of air attenuation, scatter estimation, and noise injection, which are modelled in DeepDRR for physical accuracy. We find that these calculations can lead to noise-like patterns, reduction in contrast, or lack in robustness. By removing these calculations, we make CT2Xray fast enough to be used for online training and end-to-end differentiable. Furthermore, as the tissue volume is a combination of many materials, $\mu(tissue, E)$ may inaccurately represent the attenuation coefficients of all tissues. Further separating tissue material is an intractable problem, thus we introduce a weight coefficient $\omega_{tissue}$ for $\mu(tissue, E)$ to modulate the relative contribution of bone and tissue attenuation to the final output, and provide an extra degree of freedom. As shown in Fig. \ref{fig:projector}, the output of CT2Xray is much more realistic than traditional DRR images. For more details on the implementation of CT2Xray, please refer to the supplemental material section.


\textbf{Single X-ray Backprojector}.
While CT2Xray enables a transformation from a CT volume to an X-ray image, an inverse function for CT2Xray is needed to transform a single X-ray image to a CT volume. Such a 2D-to-3D transformation is clearly ill-posed; however, we can formulate an inverse function of the forward projector to properly place the input X-ray image in 3D and ease the challenge in recovering the same X-ray image through a data-driven way. We name such an inverse function the \textit{single X-ray backprojector}. Following the formulation of general 3D backprojection algorithm for many X-ray images, e.g. as described in \cite{KINAHAN2004421}, we use a simplified version for single X-ray backprojector, where
\begin{equation} \label{eq:bp}
 V^{T}_{BP}(y) = BP(I(x)) = 
 \begin{cases}
   \frac{I(x)}{\lvert \bm{l}(x) \rvert \Delta p}, &\text{if} ~~ Ty \in \bm{l}(x),\\
     0, &\text{otherwise. }
 \end{cases}
\end{equation}
By substituting $V^{T}_{BP}$ in (\ref{eq:bp}) into $V_{CT}$ in (\ref{eq:drr}), the same $I$ is recovered under view $T$, hence we denote $V^{T}_{BP}$ obtained in this way as the backprojection of $I$ at view $T$. While the same image-wise consistency does not generally apply to CT2Xray, we show that by adding a CNN to complement the single X-ray backprojector, such consistency can be well approximated due to geometric consistency.

\subsection{XraySyn}
\begin{figure*}[htb]
\centering
\includegraphics[width=\textwidth]{imgs/XraySyn_net_new.png}
\caption{The proposed network structure of XraySyn and XraySyn+. XraySyn is shown in the grey area, which incorporates our proposed CT2Xray and single image backprojection operators to assist the geometric transformation between the X-ray and CT domain. XraySyn+ further incorporates XraySyn by projecting the estimated volume $V_{XS}$ onto a manifold discovered by a pre-trained 3D PGGAN on chest CTs to obtain a more detailed $V_{XS+}$.}
\label{fig:network}
\end{figure*}

The single X-ray backprojector produces a $V^{T}_{BP}$ from the input X-ray view $I^{T}$, and CT2Xray produces an output X-ray view $I^{T^{'}}$ from $V_{CT}$; to complete the end-to-end X-ray view synthesis process, a function $G$ is needed to recover $V_{CT}$ from $V^{T}_{BP}$. Mathematically, the overall view synthesis process can be expressed as:
\begin{equation} \label{eq:xraysyn}
    V_{XS} = G(BP(I^{T}_{in}, T); \theta), ~~ I^{T^{'}}_{XS} = CT2Xray(V_{XS},T^{'}),
\end{equation}
where $\theta$ represents the parameters in the CNN-based function $G$. %As a 2D UNet structure is often used in image-to-image tasks, e.g. pix2pix, 
We use a 3D UNet \cite{DBLP:conf/miccai/CicekALBR16} to construct $G$. Leveraging the geometrically consistent translation between the 2D and 3D domains, the losses for training $G$ are defined as:
\begin{align}\label{eqn:loss}
    \mathcal{L}_{G} &= \lambda_{CT}\mathcal{L}^{G}_{CT} + \lambda_{xray}\mathcal{L}^{G}_{xray} + \lambda_{GAN}\mathcal{L}_{LSGAN}, 
\end{align}
where $\lambda_{CT}$, $\lambda_{xray}$, and $\lambda_{GANs}$ are weights for different losses. $\mathcal{L}^{G}_{CT}$ and $\mathcal{L}^{G}_{xray}$ are defined as:
\begin{align}\label{eqn:loss2}
\mathcal{L}^{G}_{xray}=\lambda_{in}\lVert I^{T}_{XS} - I^{T}_{in} \rVert_1 + \lambda_{new}\lVert I^{T^{'}}_{XS} - I^{T^{'}}_{gt} \rVert_1 \\
\mathcal{L}^{G}_{CT} = \lVert V_{XS} - V_{CT} \rVert_1, 
\end{align}
where $\lambda_{in}$ and $\lambda_{new}$ are perspective weights for the input X-ray view and the new X-ray view. The LSGAN loss for training XraySyn is defined as:
\begin{align*}
\mathcal{L}_{LSGAN}(D)=\mathbb{E}(D(V_{CT})-1)^2 + \mathbb{E}(D(V_{XS})-0)^2\\
\mathcal{L}_{LSGAN}(G)=\mathbb{E}(D(V_{XS})-1)^2,
\end{align*}
where $D$ is a 3D discriminator network.% for more network details please refer to Supplemental Material.


\textbf{XraySyn+}. 
Recovering a $V_{CT}$ with anatomically realistic details from $V^{T}_{BP}$ is very difficult
due to the challenging nature in 2D-to-3D inversion. The conditional GAN setup as described in Eq. \ref{eqn:loss}, when dominated by the pixel and voxel-wise losses, inhibit the ability of GAN to generate fine and realistic details. Unfortunately, anatomical details like bones are disproportionally presented in X-ray images compared to their volume size due to their high material density and attenuation rate, and an incomplete recovery of such details leads to unrealistic X-ray images.

In order to enhance XraySyn's ability in generating complete and realistic anatomic details, we propose an alternative version of XraySyn called XraySyn+. XraySyn+ leverages recent advances in unconditional GANs, specifically with PGGAN, which are able to produce very realistic images. We first training a 3D variant of PGGAN that can generate CT volumes. A 3D encoder $F$ is then introduced to project $V_{XS}$ onto the manifold spanned by the PGGAN. The resulting X-ray projections and CT volumes are described as:
\begin{align*}
V_{XS+} = PGGAN(F(V_{XS}; \phi); \psi)\\
I^{T^{'}}_{XS+} = CT2Xray(V_{XS+},T^{'}),
\end{align*}
where $\phi$ and $\psi$ are parameters for $F$ and the PGGAN, respectively. The losses for training $F$ is defined as:
\begin{align}\label{eqn:loss+}
    \mathcal{L}_{F} &= \lambda_{CT}\mathcal{L}^{F}_{CT} + \lambda_{xray}\mathcal{L}^{F}_{xray} + \lambda_{code}\mathcal{L}_{code},
\end{align}
where $\mathcal{L}^{F}_{CT}$ and $\mathcal{L}^{F}_{xray}$ are as similarly defined in (\ref{eqn:loss2}) using $V^{T}_{XS+}$ and $I^{T^{'}}_{XS+}$. A code consistency loss $\mathcal{L}_{code}$ is introduced to encourage the projections of $V_{XS}$ and the groundtruth CT volume to be similar. It is defined as:
\begin{align}\label{eqn:code_consis}
    \mathcal{L}_{code} &= \lVert F(V_{XS+}; \phi) - F(V_{CT}; \phi) \rVert_2
\end{align}
Lastly, similar to the hybrid method described by Zhu et al. \cite{DBLP:conf/eccv/ZhuKSE16}, the latent code $z_{Recon}$ is updated for 1000 steps for each individual volume by the solving for the following optimization problem:
\begin{align}\label{eqn:optim}
    \argmin_{z} \lVert CT2Xray(PGGAN(z), T) - I^{T}_{in} \rVert_1,
\end{align}
where $z$ is initialized with $F(V_{XS+}; \phi)$. 


%Similar to the forward projector, the single image backprojector can be run at real time through the use of GPU.
%Further note that this is unlike the filtered backprojection algorithm commonly used in CT reconstruction, as only a single image is used.

%TODO: add the 3D UNet part using the above formulations.




%As $\mu(m, E)$ is a scalar value measured by \cite{hubbell1995tables}, The main challenge to making the entire pipeline differentiable is the calculations of $t(m)$. 




% As shown in Fig. \ref{fig:projector}, the algorithm first separates the lung CT $V_{CT}$ into a bone and tissue volume, $V_{bone}$ and $V_{tissue}$, to allow attenuation calculation of different materials. This step can be performed manually, through a dedicated segmentation algorithm, or Housefield Unit(HU) thresholding. Forward projection is performed individually over $V_{bone}$ and $V_{tissue}$ to obtain $I_{bone}$ and $I_{tissue}$, which represents the thickness of the material during every path. The attenuation rates of $I_{bone}$ and $I_{tissue}$ are calculated over a spectrum of 151 energy states\cite{hubbell1995tables}, where higher energy leads to less attenuation. The weighted sum of bone and tissue attenuation $\mu_{bone}$ and $\mu_{tissue}$ goes through the exponential decay model described as

% \begin{align}
%     I_{atten}^{i} = e^{\mu_{bone}^{i} + \omega_{tissue} \times \mu_{tissue}^{i}}, I_{Xray}^{'} = \sum_{i} I_{atten}^{i}
% \end{align}

% where $i$ represents the different energy state, and $I_{Xray}^{'}$ represents the X-ray image in terms of attenuation rate. In addition to calculating gradients for the entire pipeline to enable end-to-end training, CT2Xray discards the calculation of air attenuation, scatter estimation, and noise injection in DeepDRR to reduce the computation costs. While these processes realistically model the X-ray imaging physics, we find that they minimally affect the image quality. Furthermore, as $V_{tissue}$ is a combination of many materials, we find that $\mu_{tissue}$ may inaccurately represent the attenuation contribution of tissues. Since further separating tissue material is an intractable problem, we introduce a weight parameter $\omega_{tissue}$ to modulate between the relative contribution of bone and tissue attenuation to the final output. Lastly, clinical X-ray images are printed as inverted versions of $I_{Xray}^{'}$ and oftentimes clipped into certain dynamic range for better regional contrast; this process is also simulated in CT2Xray as the last stage in Fig. \ref{fig:projector}, and can be described as:
% \begin{align}
%     I_{Xray} = Clip(max(I_{Xray}^{'}) - I_{Xray}^{'}, floor, ceiling),
% \end{align}
% where the floor and ceiling values depends on the intended dynamic range.





==> supplemental_material_old.tex <==
\section{Supplemental Material}


\subsection{Comparison of CT2Xray and DeepDRR}
\input{imgs/supplemental/versus}
\input{imgs/supplemental/tissue_weight}
While CT2Xray is inspired by DeepDRR, it is improved in many aspects in order to work on the task of X-ray view synthesis. Beyond the ability to propagate gradients, we show here the other aspects of improvements of CT2Xray, namely in speed and flexibility. 

The DeepDRR pipeline involves segmentation of a CT volume into three materials: bones, tissues, and air. Each material is forward projected to generate $t_{bone, tissue, air}$ and undergoes attenuation calculation. A CNN-based scatter estimation and a Poisson noise are added on top of the attenuation calculation. As shown in Fig. \ref{fig:versus}, we find that the scatter estimation CNN is not robust enough for general usage, and finetuning it requires MC simulation of X-ray images, which is infeasible to scale. Based on the results from DeepDRR, scatter estimation contributes relatively little to the overall image quality; therefore, we discard the scatter estimation. We also discard the calculation of $t_{air}$, as we find that the simulation without it bares more semblance to real X-ray images found in CheXpert, where the contrast between bone and air is significantly higher. Overall, CT2Xray is about five times faster than DeepDRR.


Since tissues consist of a wide range of materials, each with different attenuation rate, and the current CT2Xray pipeline considers all tissue as one material, there exists discrepancies between the generated X-ray image and a real X-ray image. Specifically, there is no way to modulate the contribution of $\mu_{tissue}$ in the final X-ray output when $\mu_{tissue}$ is either over-estimated or under-estimated. We therefore introduce a weight $\omega_{tissue}$ to fill this need. As shown in Fig. \ref{fig:tissue_weight}, when $\mu_{tissue}$ is clearly over-estimated for the heart region, we can lower $\omega_{tissue}$ to make it much more similar to the real X-ray input.





==> tables/ablation.tex <==
\begin{table*}[t!]
\small
\centering 
\begin{tabular}{| c|c|ccc c |}
\hline
PSNR/SSIM & Loss &Volume & X-ray Orig & X-ray View 1 &  X-ray View 2 \\
% \hline
% \multirow{ 2}*{Bicubic}  & x4 &  &  &  &  &   \\
%  & x6 &  &  &  &  &  \\
\hline

X2CT-CNN\cite{DBLP:conf/cvpr/YingGMWWZ19} & $\mathcal{L}_{CT}+\mathcal{L}_{xray}$&17.57/0.5327 & 20.34/0.6787 & 19.75/0.6797 & 18.70/0.7597   \\
$\textrm{XraySyn}^{Refine}$ & $\mathcal{L}_{CT}+\mathcal{L}_{xray}$& 17.86/0.5505 & 27.05/0.9234 & 23.14/0.8175 & 18.32/0.7480\\
\hline
2D Encoder & $\mathcal{L}_{CT}+\mathcal{L}_{xray}$& 16.32/0.4360 & 18.90/0.5836 & 18.81/0.5903 & 17.98/0.6856\\
$\textrm{XraySyn}^{Refine}_{GAN}$ & $\mathcal{L}_{CT}+\mathcal{L}_{xray}+\mathcal{L}_{GAN}$& 16.91/0.4434 &23.14/0.7911 &21.34/0.7098& 18.15/0.6869\\
XraySyn & $\mathcal{L}_{CT}+\mathcal{L}_{xray}+\mathcal{L}_{code}$& 16.61/0.4522& 22.82/0.7310&21.33/0.7068 & 18.61/0.7113 \\
\hline



\hline
\end{tabular}
\vspace{-1pt}
\caption{Ablation study of XraySyn against alternative methods with quantitative evaluations. The quantitative metrics are calculated based on test data from LIDC-IDRI\cite{armato2011lung}}
\label{tab:ablation_table}
\vspace{-1pt}
\end{table*}

==> tables/modified_ablation.tex <==
\begin{table*}[htb!]
\small
\centering 
\setlength\tabcolsep{1.5pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{Metrics} & 2D Refiner & 2D Encoder & X2CT-CNN & $\textrm{XraySyn}^{v1}$ & $\textrm{XraySyn}^{v2}$ & $\textrm{XraySyn}^{v3}$ & XraySyn+\\
% \hline
% \multirow{ 2}*{Bicubic}  & x4 &  &  &  &  &   \\
%  & x6 &  &  &  &  &  \\
\hline

Orig &Xray &\diagbox[innerwidth=5em, height=1.1em]{}{}& 18.90/0.584 & 20.34/0.679&22.13/0.814 &\textbf{27.05/0.923} & \underline{23.14/0.791} &22.82/0.731\\
\hline
Orig &Bone &\diagbox[innerwidth=5em, height=1.1em]{method}{view} & 17.40/0.378& 16.02/0.206&18.47/0.491 & \textbf{19.61}/0.544&19.04/\textbf{0.552} &\underline{19.24}/\underline{0.547}\\
\hline
Orig &Tissue &\diagbox[innerwidth=5em, height=1.1em]{}{} & 19.14/0.622&19.49/0.692 & \underline{21.20}/\textbf{0.766} & \textbf{21.58}/\underline{0.753}& 20.78/0.700 &20.71/0.699\\
\hline
Orig &FID &\diagbox[innerwidth=5em, height=1.1em]{}{} &\underline{0.593}& 2.388& 0.965& 0.776& 1.025 &\textbf{0.564}\\
\hline
Rand. &Xray &\underline{23.30/0.783}& 18.81/0.582& 20.01/0.675& 21.52/0.782& \textbf{24.99/0.860}& 22.62/0.766&22.13/0.717\\
\hline
Rand. &Bone &\diagbox[innerwidth=5em, height=1.1em]{}{} & 17.32/0.378& 15.90/0.204& 18.02/0.466& \textbf{19.03}/0.513& 18.96/\underline{0.530}&\underline{18.99}/\textbf{0.537}\\
\hline
Rand. &Tissue &\diagbox[innerwidth=5em, height=1.1em]{}{} & 19.22/0.625& 19.54/0.693& \underline{21.07/0.758}& \textbf{21.40/0.754}& 20.78/0.705&20.64/0.698\\
\hline
Rand. &FID & 1.779&\underline{0.585}& 2.383& 1.003& 0.873& 1.134&\textbf{0.555}\\

\hline


% X2CT-CNN\cite{DBLP:conf/cvpr/YingGMWWZ19} & $\mathcal{L}_{CT}+\mathcal{L}_{xray}$&17.57/0.5327 & 20.34/0.6787 & 19.75/0.6797 & 18.70/0.7597   \\
% $\textrm{XraySyn}^{Refine}$ & $\mathcal{L}_{CT}+\mathcal{L}_{xray}$& 17.86/0.5505 & 27.05/0.9234 & 23.14/0.8175 & 18.32/0.7480\\
% \hline
% 2D Encoder & $\mathcal{L}_{CT}+\mathcal{L}_{xray}$& 16.32/0.4360 & 18.90/0.5836 & 18.81/0.5903 & 17.98/0.6856\\
% $\textrm{XraySyn}^{Refine}_{GAN}$ & $\mathcal{L}_{CT}+\mathcal{L}_{xray}+\mathcal{L}_{GAN}$& 16.91/0.4434 &23.14/0.7911 &21.34/0.7098& 18.15/0.6869\\
% XraySyn & $\mathcal{L}_{CT}+\mathcal{L}_{xray}+\mathcal{L}_{code}$& 16.61/0.4522& 22.82/0.7310&21.33/0.7068 & 18.61/0.7113 \\


\end{tabular}
\caption{Ablation study of our proposed methods against alternative implementations. The quantitative metrics are calculated based on test data from LIDC-IDRI\cite{armato2011lung}. 2D Refiner is a purely image-to-image approach and does not involve generation of bone and tissue, therefore respective metrics are omitted.} 
\label{tab:ablation_table}

\vspace{-1em}
\end{table*}

==> tables/new_ablation.tex <==
\begin{table*}[htb!]
\small
\centering 
\setlength\tabcolsep{1.5pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
% & view/method & \multicolumn{3}{|c|}{$T$} & \multicolumn{3}{|c|}{$T^{'}$}\\
\multirow{5}{*}{Simulated}  & \diagbox[innerwidth=6em, height=2em]{Method}{View} & $I^{T}_{\textrm{CT}}$ & $t^{T}_{\textrm{bone}}$ & $t^{T}_{\textrm{tissue}}$ & $I^{T^{'}}_{\textrm{CT}}$ & $t^{T^{'}}_{\textrm{bone}}$ & $t^{T^{'}}_{\textrm{tissue}}$ \\
\cline{2-8}
& 2D Refiner & \diagbox[innerwidth=5em, height=1.1em]{}{} & \diagbox[innerwidth=5em, height=1.1em]{}{} & \diagbox[innerwidth=5em, height=1.1em]{}{} & 21.09/0.801 & \diagbox[innerwidth=5em, height=1.1em]{}{} & \diagbox[innerwidth=5em, height=1.1em]{}{}\\
\cline{2-8}
& X2CT & 20.44/0.755 & 15.99/0.451 & 19.57/0.711 & 20.20/0.750 & 16.12/0.450 & 19.38/0.703\\
\cline{2-8}
& 3DPN-DRR & 21.05/0.925 & \diagbox[innerwidth=5em, height=1.1em]{}{} & \diagbox[innerwidth=5em, height=1.1em]{}{} & 19.79/0.867 & \diagbox[innerwidth=5em, height=1.1em]{}{} & \diagbox[innerwidth=5em, height=1.1em]{}{}\\
\cline{2-8}
& 3DPN & 29.49/0.961 & 22.30/0.814 & 24.40/0.866 & 27.22/0.929 & 21.63/0.780 & 24.27/0.860\\
\hline
\multirow{4}{*}{Real} & \diagbox[innerwidth=6em, height=2em]{Method}{View} & \multicolumn{3}{c|}{$I^{T}_{\textrm{final}}$} & \multicolumn{3}{c|}{$I^{T^{'}}_{\textrm{final}}$(FID only)}\\
% \cline{2-8}
% & 3DPN-DRR &  \multicolumn{3}{c|}{}  & \multicolumn{3}{c|}{} \\
\cline{2-8} 
& 3DPN &  \multicolumn{3}{c|}{22.75/0.819}  & \multicolumn{3}{c|}{1.09} \\
\cline{2-8}
& $\textrm{XraySyn}^{\textrm{no}\mathcal{M}}$ &  \multicolumn{3}{c|}{28.42/0.857}  & \multicolumn{3}{c|}{0.375} \\
\cline{2-8}
& XraySyn & \multicolumn{3}{c|}{30.33/0.865}  & \multicolumn{3}{c|}{0.319} \\

\hline

\end{tabular}
\caption{Ablation study of our proposed methods against alternative implementations. Note that 3DPN-DRR and 2D Refiner do not use CT2Xray, therefore are without metrics for $t_{\textrm{bone}}$, $t_{\textrm{tissue}}$. $I^{T}_{\textrm{CT}}$ for 2D Refiner is trivially generated as $I^{T}_{\textrm{in}}$. PSNR/SSIM metrics are provided when groundtruth is available, otherwise FID score is reported. The best performing metrics are \textbf{bold}, the second best metrics are \underline{underlined}.} 
\label{tab:ablation_table}

\vspace{-1em}
\end{table*}
